What Does the Chart Say? Grouping Cues Guide Viewer Comparisons and Conclusions in Bar Charts

Reading a visualization is like reading a paragraph. Each sentence is a comparison: the mean of these is higher than those; this difference is smaller than that. What determines which comparisons are made first? The viewer's goals and expertise matter, but the way that values are visually grouped together within the chart also impacts those comparisons. Research from psychology suggests that comparisons involve multiple steps. First, the viewer divides the visualization into a set of units. This might include a single bar or a grouped set of bars. Then the viewer selects and compares two of these units, perhaps noting that one pair of bars is longer than another. Viewers might take an additional third step and perform a second-order comparison, perhaps determining that the difference between one pair of bars is greater than the difference between another pair. We create a visual comparison taxonomy that allows us to develop and test a sequence of hypotheses about which comparisons people are more likely to make when reading a visualization. We find that people tend to compare two groups before comparing two individual bars and that second-order comparisons are rare. Visual cues like spatial proximity and color can influence which elements are grouped together and selected for comparison, with spatial proximity being a stronger grouping cue. Interestingly, once the viewer grouped together and compared a set of bars, regardless of whether the group is formed by spatial proximity or color similarity, they no longer consider other possible groupings in their comparisons.

==> BackupTex/backup.tex <==
Bar visualization has limitation on shape. Investigate shape with scatter.
Also we saw that color was weak in bars compared to spatial and size grouping, what about in comparison to shape? 



Scatter plot also provides on additional dimension. 

% X -> Y conclusions 
In many plots on the Cartesian plane,
the x value on the horizontal axis has some role in determining or
influencing the y value on the vertical axis. A high school or college
student is likely to internalize these conventions; when viewing a plot
in the Cartesian plane the natural assumption is that the variable on the
horizontal axis is having some 

The example should be a comparison of the means of group, because it's the most common and correspond to many decision criteria (e.g., one class is better) . Scatterplots enable viewers to visually aggregate data is advantagesous, because you don't need to know the viewers needs, plus you are providing a natural combination of the statistics with details and trends. 

In these scatterplot mean comparison tasks, we know that stronger cues (color) outperforms weaker ones (shape), and combining cues redundantly (color + shape) does not improve performance. Irrelevant cues do not degrade performance - so class is separated by color, but adding random shapes to each color doesn't influence mean comparisons \cite{gleicher2013perception}.


\begin{table}[h]
\renewcommand{\arraystretch}{1.1} \small \centering
  \caption{Scatter Odds Ratio to draw a category of conclusion for each rank }
  \begin{tabular}{lllll}
  \newline \\ {\bf Rank} & {\bf Category} & {\bf Color} & {\bf Shape} & {\bf Both} & {\bf None} \\ \hline 
\multirow{6}{4.5em}{First Conclusion} & 
\rowcolor{gray!25} main effect & \textbf{1.00} & 0.51*** & 0.00*** &  0.00 \\
 & pair-wise & 0.02 & 0.00 & 0.00 & \textbf{2.52e+39***} \\
 & \rowcolor{gray!25} superlative & 0.22 & 0.00*** & \textbf{6.60***} & 0.00\\
 & correlation & \textbf{0.08} & \textbf{0.08} & 0.00 & 0.20 \\
 & \rowcolor{gray!25} distribution & \textbf{0.04} & 0.02 & 0.02 & 0.00 \\  \hline 
 
 \multirow{6}{3em}{Second Conclusion} & 
main effect & \textbf{1.00} & 0.51*** & 0.00*** &  0.00 \\
 & \rowcolor{gray!25} pair-wise & 0.09 & 0.00 & 0.00 & 1.13e+40\\
 &  superlative & 0.25 & 0.00 & 7.5 & 0.00 \\
 & \rowcolor{gray!25}correlation & 0.09 & 0.09 & 0.00 & 0.23 \\
 & distribution & 0.07 & 0.03 & 0.04 & 0.00 \\ \hline 
 
 \multirow{6}{3em}{Third Conclusion} & 
\rowcolor{gray!25} main effect & \textbf{1.00} & 0.51*** & 0.00*** &  0.00 \\
 & pair-wise & & & & \\
 & \rowcolor{gray!25} superlative & & & & \\
 & correlation & & & & \\
 & \rowcolor{gray!25} distribution & & & & \\
    \end{tabular}
    \label{color_all}
\end{table}

% What is an effective visualization? One that gets the intended message across
Generally speakig, if a visualization is designed to share a message, but the message is not among the first take-aways an average viewer would generate, you've failed. EXAMPLE (?). 

How do we know if a visualization conveys \textit{intended} message? Commonly people use Query task - like data value extraction, understanding trends and comparing trends. Bertin introduced this \cite{bertin1983semiology,}. Although a common choice \cite{lai2016measuring, lee2016vlat}, it does not give us insight on \textit{what} people would conclude from visualization and doesn't shed light on comprehension, or whether the intended message goes across.

There has been approaches trying to get at the foundational principles to assess the effectiveness of data visualizations. 
% approaches at measuring how visualizations are effective
People made several models:

1. Saliency model or eye tracking. Based on properties of human visual system. Predict which areas of a scene have visual features (coloe, luminance) that would draw a viewers' attnetion. Such as models to predict where people would look \cite{janicke2010salience,matzen2017data,matzen2016using}, so designers can evaluate whether the visualization draws viewer attention as intended. Limitation: focus on bottom-up visual attention, which is only part of the picture. There is top-down visual attention that this cannot capture - such as viewers' goal and reasoning routines, also cannot capture what people are thinking on a higher-level, no way of knowing if the intended message goes across. 

2. Technique for Measuring Comprehension of visualizations: evaluate whether people understand it or not. There are multiple teests of graph literacy or interpretation. Standard practice is having eperts in a field to produce a test \cite{royer1981theory}. Covering the range of forms for
statistical graphics requires a large corpus of questions \cite{wainer1980test}. Recent researchers have developed an algorithmic method to generate queries to measure comprehension for statistical graphs \cite{livingston2019query}. They introduced the idea of visualization as analogy to sentences. There exist an original source visualization, and paraphrase visualizations that communicates a gist of the source visualization. Participants would determine whether the information shown in the paraphrased visualization was stated or not stated in the source graph.

% Let's instead of measuring whether visualization is effective, see what humans are doing. Use that information to inform effective design of visualizations. 
In light of these two models, we push for this reasoning model, to look at how visual element within one visualization influence the type of conclusions people tend to draw from a visualization. 

\subsection{Visual Comparison}
 GIVE A CONCRETE EXAMPLE OF AB AND WEST EAST, TO DETERMINE WHICH PRODUCT IS SELLING BETTER IN WHICH REGION, TO INFORM MARKETING OR DEVELOP NEW BUSINESS STRATEGY, ONE HAS TO COMPARE THE HEIGHT OF THE BARS ETC. USE THE PILOT BAR GRAPH AS FIGURE. 

% 1. conclusion is reached through comparison, thus comparison is important.
Gleicher \cite{gleicher2017considerations} identified the two key element in a comparison:  \textit{targets} to be compared, which are REFER BACK TO EXXAMPLE, and an action performed on the relationship among the target )similarities and differences), REFER BACK TO EXAMPLE. To come to a valid conclusion using data, it often involves the viewer looking at multiple data points - such as looking for differences between two genetic sequences, or comparing how revenue is distributed across several regions. This requires extracting relation from multiple data points.Data analysists often have to engage in such visual comparison to reach conclusions, and thus understanding how a visualization can help viewers identify targets and the relationship is critical to design effective visualizations. 

% 2. people studied comparison.
Past people have studied how visual design can better support comparison. One of the earliest line graph by William Playfair is a comparison of import and export routes between England to the East Indies to show import imbalance - much more imports from England from the East Indies than exports \cite{cleveland1984graphical}. However, most research on comparisons focus on perceptual analytic tasks, determing which visual elements are more likely to drive an accurate comparison, rather than which visual elements are more likely to be compared. 

Cleveland and McGill: position more accurate, hue less accurate when compared. \cite{cleveland1984graphical}
Face too Face: spatial arrangement strongly impacts find biggest mean and biggest range. \cite{ondov2018face}
Generating averages: stronger cues (color) outperform weaker ones (shape) in scatter plot when people are asked to compare average value of multiclass scatterplots. \cite{gleicher2013perception}


But what is the most efficient/accurate (that facilitates comparison) isn't necessarily what people would compare. Climate scientists continue to prefer using rainbow color scales to compare data magnitude in maps, although they perform much more accurately when using monotonic luminance scales (such as the Kindlmann scale) \cite{dasgupta2018effect}. 

This motivates us to extend from perceptual tasks measuring comparison accuracy to cognitive tasks to elicit preference. We extend the perceptual tasks to cognitive task. In addition to determining \textit{how} accurate people make visual comparisons, we investigate \textit{what} people are likely to compare. Through crowd-sourcing, we investigate the comparisons people most likely make from a visualizatoin. By studying what humans would generate as sentence conclusions, we can see what visual elements elicit what type of comparisons and conclusions, use that to predict human decisions with visualisations, measure graph comprehension, and design recommendation systems.


\subsection{Visual Grouping and Inference Generating}
% 1. Studying comparison is an extension of studying visual grouping. Visual grouping has been well studied in vision.
In graph comprehension, the initial step is that visual elements such as color and shape, are identified and grouped \cite{pinker1990theory}. Bottom-up factors such as spatial proximity and color similarity will influence those visual groups. (Expert viewers may have top-down, knowledge/expertise driven way of grouping, but we will not talk about it here.) 

% 2. Visual grouping then goes back to help generating inferences in visualization
People are more likely to make discrete comparisons with bar graphs, we know that \cite{carswell1993stimulus}. But what type of discrete comparisons?! Within the same bar graphs with just four data points, there are X many comparisons one could already make. 

In bar graph, Gestalt principle of proximity preidcts that viewers would encode the grouped set of bars \cite{shah1999graphs}. What if we add color to the mix? 

Verbal descriptions of the graph, if dependent on visual chunks, would differ depending on what is grouped. 

% 3. Visual grouping associated with concluding main effect / interactions in visualization
% rephrase this in terms of main effect and interaction %
In bar graphs where there is a third dimension of z-axis with legend (color encoding), peopel's description typically focus on the effect of the variable plotted on the z-axis (color) on the x-axis. So z's effect on y, moderated by x \cite{shah2011bar}. Which is the main effect of z, rather than the main effect of x. EXAMPLE Using Bar Graph, adapt from Shah and Freedman 2011. 

We will further examine how the visual grouping will influence the type of comparison (x-y, z-y, x-z)

% Hypothesis Motivaton %
\section{Hypothesis Motivation}
To achieve the broader goal of creating a computational model that captures how patterns and relations in a visualization can be expressed as sentences produced by a human, one first step is to gather information on how humans create sentences when viewing a visualization. To further simply the problem without losing external validity, we begin experimenting with simple visualizations commonly found in media and scientific journals - bar graphs and scatter plots. While many components of a visualization could be examined (see \ref{otherComponents} for a summary of the space), we focus on spatial, color and shape grouping for the scope of this paper. 

We emprically examine the intuitively-motivated guideline from Gleicher et al \cite{gleicher2011visual} to see if spatial grouping is truly the strongest visual element to elicit comparison. 

Hypothesis: visual grouping -> more likely to make comparison, 
spatial + color > spatial > color
when there is no color grouping, just spatial, people might be less likely to compare than when there is additional color grouping. 

% talk about superlative visual search a little bit - how it's a different type of search than comparison % 


\subsection{Drawing Conclusions from Visualizations}
Cite: 
https://www.mitpressjournals.org/doi/pdf/10.1162/COLI_a_00091
https://www.aclweb.org/anthology/W11-2703.pdf
(about text in visualizations)




















%% STUDY OVERVIEW %%
\section{Study Overview}
Through two crowded-sourced experiments, we create a preliminary model that would predict what comparisons an average viewer would likely produce with a given visualization. In Experiment 1, participants viewed bar charts with two binary factors (four total bars) with competing groupings of proximity, color, and size. They were the most likely to group and compare marks with similar sizes (e.g., the average of these two large values is larger than of those two small values), followed by comparing spatially proximal marks, followed by groups of the same color. In Experiment 2, participants viewed scatterplots with two binary factors (four clusters), with competing groupings across color and shape. Participants were more likely to compare groups encoded with different colors, before moving on to comparing shape. We also found an additional trend of participants more likely to compare points in a multiple-class scatterplots based on their y-values. With refinement and tests for generalizability, this model could produce firm guidelines on how to design visualizations that effectively communicate an intended pattern in data.

\subsection{Visualizing Data in This Paper}
In the spirit of the experiment, we present all of our result visualizations in two different ways so you can make different comparisons. Most of our results are visualizing several dimensions simultaneous using facet functions. For example, in Figure \ref{fig:bar_all}, the top section visualizes the data with columns grouped by underlying data relations and rows grouped by the order the sentence conclusions were generated. Each row represents one category of comparisons, following the taxonomy in section \ref{taxonomy}. The bottom section visualizes the same data, but columns are now grouped by color grouping, rows grouped by comparison categories, and each row represents the order the sentence of a specific category was produced. Also, since reading a visualization parallels reading a paragraph and to facilitate mapping between the figures and the result section, we annotated several patterns to guide you through key comparisons. 

\begin{figure}[th]
 \includegraphics[width=3.4in]{PossibleConclusions.jpg}
 \caption{Depictions of the three main categories of conclusions as well as the specific types of conclusions proximal those categories. \textit{distal group} conclusions contain comparisons across the spatially grouped data, while \textit{proximal group} conclusions contain comparisons distal the spatially grouped data. Pair-wise comparisons have additional categories, as specific conclusions may involve only the distal or only the proximal data points.}
 \label{fig:bar_categories}
\end{figure}

==> BackupTex/backup_exp1.tex <==
%% Bar Visualization Design Space%%
\begin{figure*}[th]
 \includegraphics[width=17.8cm]{BarDesignSpace.jpg}
 \caption{Design Space for Bar Graph Experiments. (a) Experiment 1a - all same color. (b) Experiment 1b - how color addition changes conclusion}
 \label{fig:exp1design}
\end{figure*}

%% EXPERIMENT 1 %%
\section{Bar Visualizations Experiments}
To investigate the effect of spatial, color and size grouping, we selected three combinations of main effects and interactions to cover six of the unique and interesting relations from the eight possibilities as shown in Figure \ref{fig:eightRelationships}, in hopes of balancing potential confound created by data relations and size grouping. We created three data sets with three different underlying relations: one data set with no main effect but an interaction (h), one with one main effect but no interaction (b/c), and one with two main effects but no interaction (a). We used the same two factors (company and region) from the pilot. Each data set is presented as a bar chart either spatially grouped by company or by region, subsequently making the size grouping either congruent or incongruent to the spatial grouping. All data sets were perturbed with some noise. Figure \ref{fig:exp1design} shows the design space.

\subsection{Data Relation, Spatial and Size Grouping}
We first investigate how spatial and size grouping affect conclusions people draw without considering color grouping, as shown in Figure \ref{fig:exp1design}(a). This experiment follows the same procedure as the pilot experiment. Participants viewed these bar charts and wrote down their top three conclusions. Power analysis based on the pilot effect sizes derived from logistic regression models suggested a target sample of 45 conclusions per category (e.g., main effects, interactions, pair-wise) would give us 80\% power to detect patterns in conclusion frequencies at alpha level of 0.05 \cite{hsieh1998simple}. Because we have no control over the conclusions a given participant would draw from a visualization, we iteratively surveyed and excluded participants on Amazon's Mechanical Turk who gave nonsensical answers or failed attention tests until we have at least 45 conclusions for each bar charts.

%% DESIGN AND PROCEDURE %%
\subsubsection{Summary Statistics on Conclusion Categories}
The conclusions come from 102 unique participants ($M_{age} = 40.02$, $SD_{age} = 9.99$, 40 females), each writing their top three conclusions (in the order of which came to mind first). After excluding the nonsensical conclusions, we ended up with 292 conclusions. As shown in Figure \ref{fig:DistributionConclusionCategory_Rank}, amongst them, most were conclusions on main effects (47.9\%), followed by pair-wise comparisons (32.2\%), with few interactions (9.59\%), superlatives (7.54\%), and others (2.74\%).

As shown in Table \ref{barRankCategoryORTable}, multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion rankings with conclusion categories suggests that people were most likely to make a main effect comparison first. For those who didn't make a main effect comparison, they were more likely to have made a pair-wise comparison than anything else ($p_{interaction} = 0.002$, $p_{superlative} = 0.001$, $p_{other} < 0.001$). By the second conclusion, people are more likely to make a main effect comparison or a pair-wise comparison than other conclusions, but the likelihood of them making main effect comparison and pair-wise comparison was not significantly different ($p = 0.74$). By the third conclusion, people became more likely to make main effect comparisons again, and similar to what they did for the first conclusion, those who didn't make a main effect comparison more likely made pair-wise comparisons ($p_{interaction} = 0.02$, $p_{superlative} = 0.004$, $p_{other} < 0.001$). More statistical details can be found in the supplementary materials.

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
\renewcommand{\arraystretch}{1.3}
  \caption{How likely did people draw these different types of conclusions compared to a main effect, for each rank. How to interpret the numbers: a value of 0.51 for pair-wise comparison under First Rank means the odds of a participant drawing a pair-wise conclusion is 0.51 that of drawing a main effect conclusion.}
  \begin{tabular}{lrrr}
  \newline \\ {\bf Category} & {\bf First Rank} & {\bf Second Rank} & {\bf Third Rank} \\ \hline 
 main & 1.00 &  1.00 & 1.00 \\ pair-wise & 0.51 & 1.08 & 0.52 \\ interaction & 0.15 & 0.26 & 0.22\\
 superlative & 0.13 & 0.21 & 0.15 \\ others & 0.07 & 0.05 & 0.04 \\
    \end{tabular}
    \label{barRankCategoryORTable}
\end{table}

\cx{Following the spirit of the paper, because people will make different comparisons based on spatial grouping of things, we also visualize Figure \ref{fig:DistributionConclusionCategory_Rank} by category and rank instead. Right here:}


\begin{figure*}[th]
 \includegraphics[width=17.8cm]{DistributionConclusionCategory_Rank.jpg}
 \caption{Conclusions by Underlying Data Relations details, visualized both by aggregating category (top) and by aggregating rank (bottom) for experiment 1a and 1b, following the spirit of the paper.}
 \label{fig:DistributionConclusionCategory_Rank}
\end{figure*}

More specifically, the prominence of pair-wise comparisons seemed to be largely driven by people more likely making pair-wise comparisons  when the underlying data depicted no main effect but an interaction, as shown in Figure \ref{fig:DistributionConclusionCategory_RankSeparatedByRank}. We take a closer look at how underlying data relations could drive the conclusions people make.

%% Results %%
\subsubsection{Data Relation}
A $\chi^2$ test of independence with Bonferroni adjustment suggests that people more likely made main effect comparisons when they viewed data depicting one main effect and no interactions, or two main effects and no interactions, compared to data depicting an interaction but no main effects ($\chi^2 = 43.69$, $p < 0.001$). Post-hoc comparisons with Bonferroni corrections revealed that they were more likely to make pair-wise comparisons when viewing data depicting an interaction but no main effects ($z = 5.92$, $p < 0.001$). They were marginally less likely to draw interaction comparisons when viewing data depicting two main effects with no interactions compared to the other two ($z = -1.82$, $p = 0.06$). 

We then look more specifically at how conclusions varied with rank for the majority of conclusions. Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with data relations further shows that people take into consideration the underlying data relation as they make comparisons of data. Table \ref{FirstConclusionOR} shows the odds ratio of participants drawing a specific comparison as their \textit{first} conclusion for each of the three data relations. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{How likely did people draw these different types of conclusions as the FIRST CONCLUSION for each data relation type. \cx{consider replace NoMainYesInt header with mini pictures}}
  \begin{tabular}{lrrr}
  \newline \\ {\bf Conclusion} & {\bf No Main Yes Int} & {\bf One Main Only} & {\bf Two Main Only} \\ 
  \hline 
 main between & 1.00 & 1.00 & 1.00 \\
 main within & 3.00 & \textbf{2.28} & \textbf{1.66} \\
 pair-wise between & 2.50 & 0.71 & 0.33 \\
 pair-wise within & \textbf{6.00} & 0.29 & 0.11 \\
 interaction between & <0.01 & 0.14 & 0.11\\
 interaction within & 2.00 & 0.29 & <0.01 \\
    \end{tabular}
    \label{FirstConclusionOR}
\end{table}

For bar charts depicting an interaction but no main effect, the majority of conclusions were pair-wise comparisons. People were the most likely to first make a within-group pair-wise comparison (and specifically, of the left group, as shown in Figure \ref{fig:exp1aMain0Int1PairwiseDetail}). Those who didn't make a within-group pair-wise comparison would likely make a within-group main effect comparison or a between-group pair-wise comparison. For their second conclusion, they switch to make either a between-group or a within-group pair-wise comparison of the right group. Very few participants made pair-wise proximity and edge comparisons (~6\%). For those who did, these comparisons were often the second or third conclusion people drew, never the first. We omit these comparisons from the detailed visualization as shown in Figure \ref{fig:exp1aMain0Int1PairwiseDetail}.

\begin{figure}[th]
 \includegraphics[width=2in]{Main0Int1_PairwiseDetail.png}
 \caption{Detail on left or right group being compared for the pair-wise comparisons for Main0 interaction 1}
 \label{fig:exp1aMain0Int1PairwiseDetail}
\end{figure}

For bar charts depicting one main effect and no interaction, the majority of conclusions were main-effect comparisons. People were the most likely to make within-group main comparisons as their first conclusion. We can see from Figure \ref{fig:DistributionConclusionCategory_Rank} that, in fact, participants mostly make within-group main effect comparisons for their second and third comparisons as well. Those who didn't make main-effect comparisons mostly made pair-wise between-group comparisons. 

For bar charts depicting two main effects and no interaction, people likely first made a within-group main effect comparison. For their second conclusion, they either switched to make a between-group main effect comparison, or made a pair-wise comparison, as shown in Figure \ref{fig:DistributionConclusionCategory_Rank}. Different from those who viewed bar charts depicting one main effect, participants who viewed bar charts depicting two main effects were equally likely to make between-group and within-group pair-wise comparisons. 

\begin{figure}[th]
 \includegraphics[width=3.4in]{Bar_1111_SizeGrouping.png}
 \caption{SizeGrouping}
 \label{fig:exp1aSizeGrouping}
\end{figure}

\subsubsection{Size Grouping}
As previously mentioned in section \ref{insightFromPilot}, both the underlying data relation (whether there exists main effect/interaction in the data or not) and size grouping could influence the conclusions people draw. We discuss in depth two scenarios to further titrate the effect of size grouping and underlying data relations.

% Keeping data relation the same, look at size grouping
The first scenario is to hold underlying data relation constant and compare two size grouping: one congruent with spatial grouping such that the bars with similar height were also spatially placed together, and one incongruent with spatial grouping such that the bars with dissimilar sizes were spatially placed together, as shown in the first two columns in Figure \ref{fig:exp1aSizeGrouping}. Both bar charts depict one salient main effect of company, but by either grouping the factors by company (A,B) or by region (East, West), size grouping changes to be either congruent (first column of Figure \ref{fig:exp1aSizeGrouping}) or incongruent (second column of Figure \ref{fig:exp1aSizeGrouping}) with spatial grouping. 

As shown in Figure \ref{fig:exp1aSizeGrouping}(top), when size and spatial grouping are congruent, we see that most people tended to conclude a within-group main effect comparison between the two spatially separated group. When size and spatial grouping are incongruent, most people still made within-group main effect comparisons, which compared the two spatially separated groups. Interestingly, compared to the size-spatial congruent condition, more people made pair-wise conclusions and fewer people made main effect conclusions ($\chi^2 = 6.26$, $p = 0.04$). in the size-spatial incongruent condition. 

A closer look at the specific pair-wise comparisons participants made (as shown in the middle two columns in Figure \ref{fig:exp1aPairWise}) demonstrates that people tend to start with a between-group pair comparison of the two tallest bars (in this case, East A and West A), then switching to a between-group comparison of the two-shortest bars (East B and West B).  

% Keeping size grouping the same, change data relation
The second scenario is to hold size grouping the same but change underlying data relation. Specifically, we compare the bar chart that depicts one salient main effect, grouped by region, and the bar chart that depict two salient main effects, grouped by company (as shown in the last two columns in Figure \ref{fig:exp1aSizeGrouping}.

The pattern of conclusions people tend to draw was similar between these two charts. Overall, people were just as likely to draw main effects, and just as likely to draw pair-wise comparisons between these two charts ($\chi^2 = 2.33$, $p = 0.31$). A closer look at the specific pair-wise comparisons people made when viewing the two main effect bar chart demonstrates that people drew similar types of conclusions when size grouping is held constant. Similar to that with the one main effect bar chart, people tend to start with a between-group pair comparison of the two tallest bars and then switching to a between-group comparison of the two-shortest bars. 

\begin{figure}[th]
 \includegraphics[width=3.4in]{Bar_1111_PairWiseDetails.png}
 \caption{Details about what ppl did for the pair-wise comparisons}
 \label{fig:exp1aPairWise}
\end{figure}

\subsubsection{Discussion}
Underlying data relation influences the main effect comparisons people make, where as the size grouping influences the pair-wise comparisons people make. In other words, the same underlying data relation would elicit similar main-effect comparisons, while the same size grouping would elicit similar pair-wise comparisons. 

When the underlying data depicts no main effect but an interaction, people tend to not make main-effect conclusions. When the underlying data depicts one main effect, people likely would first do a main effect comparison between the two spatially grouped levels. When the underlying data depicts two main effects, people alternate between the within-group and the between-group main effect comparisons, first doing a within-group main effect comparison between the two spatially grouped levels, followed by a between-group main effect comparison between the two levels not spatially grouped. 

Holding the underlying data relations consistent, size-grouping interacts with the effect of underlying data relations such incongruent size-spatial grouping leads to more pair-wise comparisons. When the size grouping of the data is congruent to the spatial grouping, few people draw pair-wise conclusions, focusing only on the main-effect comparison congruent with size grouping. 

% Aggregated Comparison by Size Grouping (4400, 4141, 4321, 4004)
Overall, by aggregating size grouping, we see that people tend to draw the within-group conclusions comparing the two spatially separated groups when spatial grouping is congruent with size grouping, as shown in the left most column in Figure \ref{fig:exp1aMagnitudeMain}. As the size grouping become more and more incongruent with spatial grouping, people became more likely to draw a balance amount of both within-group and between-group conclusions. This shows a competition between spatial and size grouping, suggesting both are of equal strength and both drive what a viewer would conclude. More specifically, looking at Figure \ref{fig:exp1aMagnitudeMain}, if spatial grouping is the stronger driver, you would expect participants to always make within-group main comparisons. If size-grouping is the stronger driver, you would expect participants to always make between-group main comparisons when the tall and short bars alternate in the chart. 

\begin{figure}[th]
 \includegraphics[width=3.4in]{Bar_1111_MagnitudeMain.png}
 \caption{How size grouping change the balance between the within-group and between-group conclusions people drew. Error bar shows standard error. }
 \label{fig:exp1aMagnitudeMain}
\end{figure}

% discussion of potential confound
In the bar charts tested so far, we noticed that participants tend to draw conclusions starting from the left of the visualization. In bar charts depicting no main effect but an interaction (the bars were in the order of tall, short, short, tall), the majority of the people did pair-wise comparisons of the two bars on the left. In bar charts where size and spatial groupings were incongruent (the bars were in the order of tall, short, tall, short), participants drew pair-wise comparisons of the tallest two bars, one of which being the left-most. We have yet to tease apart whether this was driven by a tendency to focus on the tallest bars or to start from the left of the visualization. Experiment 1b investigate this position-size confound to further dissect how spatial arrangement and size grouping interacts to influence the conclusions people draw.

\subsection{Experiment 1b Position-Size Investigation}
We introduce two new 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment 1c Color Grouping}
We observed a competition between spatial and size grouping in Experiment 1a. We further investigate how color grouping interacts with spatial and size grouping by incorporating a color dimension in the bar charts, as shown in Figure \ref{fig:exp1design}b. The color is either mapped onto region or company, making it either congruent or incongruent with spatial grouping. Congruent color-spatial mapping means the spatially approximate two bars share the same color (e.g., grey, grey, white, white), while incongruent color-spatial mapping means the spatially approximate two bars have different colors (e.g., grey, white, grey, white). This experiment follows the same procedure as all previous experiments.

\subsubsection{Summary Statistics on Conclusion Categories}
The conclusions come from 210 unique participants ($M_age = 40.91$, $SD_age = 9.95$, 85 females). After excluding the nonsensical conclusions, we ended up with 605 conclusions. Similar to Experiment 1a, most conclusions were main effects(44.1\%), followed by pair-wise comparisons (31.7\%), with few interactions (12.7\%), superlatives (6.94\%), and others (4.47\%). 

As shown in Figure \ref{fig:DistributionConclusionCategory_Rank}b, participants who viewed the bar charts with the additional color mapping seem to follow the same pattern as those that viewed the bar charts without the color mapping. They were more likely to make main effect comparisons for data depicting one main effect and no interaction, and data depicting two main effects and no interaction. When they viewed data depicting no main effect but an interaction, they were equally likely to make main effect comparisons and pair-wise comparison at first, but shifting to make pair-wise comparisons more by their second and third conclusions. Comparing Figure \ref{fig:DistributionConclusionCategory_Rank}a and \ref{fig:DistributionConclusionCategory_Rank}b suggests that there is no significant effect of color mapping on the overall conclusion type or ranking order ($\chi^2 = 6.28$, $p = 0.18$), such that the conclusions people draw follows the same pattern between congruent color-spatial mapping and incongruent color-spatial mapping. 

\subsubsection{Interaction of Color, Spatial, and Size Grouping}
We combine the data from this experiment to that of Experiment 1a to investigate the effect of color on the comparisons viewers would make when viewing a visualization. 

%% DISCUSSION %%
\subsection{Discussion}
interesting: heuristic erros where they look at the left most bar and made more general claim than they should "East is bigger (when it's not actually" - see coding page for heuristic error. Cite Elsie's thing about heuristics

\begin{figure*}[th]
 \includegraphics[width=17.8cm]{DataRelation_ConclusionComparison.jpg}
 \caption{Did participant make a between group or a within group comparison?}
 \label{fig:DataRelationAll}
\end{figure*}


\subsection{Sentence Conclusions in Visualizations}




% 2. Visual grouping then goes back to help generating inferences in visualization
People are more likely to make discrete comparisons with bar graphs, we know that \cite{carswell1993stimulus}. But what type of discrete comparisons?! Within the same bar graphs with just four data points, there are X many comparisons one could already make. 

In bar graph, Gestalt principle of proximity preidcts that viewers would encode the grouped set of bars \cite{shah1999graphs}. What if we add color to the mix? 

Verbal descriptions of the graph, if dependent on visual chunks, would differ depending on what is grouped. 

% 3. Visual grouping associated with concluding main effect / interactions in visualization
% rephrase this in terms of main effect and interaction %
In bar graphs where there is a third dimension of z-axis with legend (color encoding), peopel's description typically focus on the effect of the variable plotted on the z-axis (color) on the x-axis. So z's effect on y, moderated by x \cite{shah2011bar}. Which is the main effect of z, rather than the main effect of x. EXAMPLE Using Bar Graph, adapt from Shah and Freedman 2011. 

We will further examine how the visual grouping will influence the type of comparison (x-y, z-y, x-z)


%subsection{Motivation}
We hypothesize to see varying degree of influence of proximity, color, and shape grouping cues on guiding viewer conclusions. When 

With proximity being the stronger grouping cue, followed by color, and shape, 

Cite: 
https://www.mitpressjournals.org/doi/pdf/10.1162/COLI_a_00091 (Summarizing Information Graphics Textually)

https://www.aclweb.org/anthology/W11-2703.pdf
(A Corpus of Human-written Summaries of Line Graphs)


Based on psych litertature, we  hypothesize to 



In bar charts, 

We emprically examine the intuitively-motivated guideline from Gleicher et al \cite{gleicher2011visual} to see if spatial grouping is truly the strongest visual element to elicit comparison. 

Hypothesis: visual grouping -> more likely to make comparison, 
spatial + color > spatial > color
when there is no color grouping, just spatial, people might be less likely to compare than when there is additional color grouping. 


We extend the perceptual tasks to cognitive task. In addition to determining \textit{how} accurate people make visual comparisons, we investigate \textit{what} people are likely to compare. Through crowd-sourcing, we investigate the comparisons people most likely make from a visualizatoin. By studying what humans would generate as sentence conclusions, we can see what visual elements elicit what type of comparisons and conclusions, use that to predict human decisions with visualisations, measure graph comprehension, and design recommendation systems.

% talk about superlative visual search a little bit - how it's a different type of search than comparison % 

\subsection{Additional Consideration of Color Grouping}
We observed a competition between spatial and size grouping in Experiment 1a. We further investigate how color grouping interacts with spatial and size grouping by incorporating a color dimension in the bar charts, as shown in Figure \ref{fig:exp1design}b. The color is either mapped onto region or company, making it either congruent or incongruent with spatial grouping. Congruent color-spatial mapping means the spatially approximate two bars share the same color (e.g., grey, grey, white, white), while incongruent color-spatial mapping means the spatially approximate two bars have different colors (e.g., grey, white, grey, white). This experiment follows the same procedure as all previous experiments.

\subsubsection{Summary Statistics on Conclusion Categories}
The conclusions come from 210 unique participants ($M_{age}$ = 40.91, $SD_{age}$ = 9.95, 85 females). After excluding the nonsensical conclusions, we ended up with 605 conclusions. Similar to Experiment 1a, most conclusions were main effects(44.1\%), followed by pair-wise comparisons (31.7\%), with few interactions (12.7\%), superlatives (6.94\%), and others (4.47\%). 

As shown in Figure \ref{fig:bar_all}b, participants who viewed the bar charts with the additional color mapping seem to follow the same pattern as those that viewed the bar charts without the color mapping. They were more likely to make main effect comparisons for data depicting one main effect and no interaction, and data depicting two main effects and no interaction. When they viewed data depicting no main effect but an interaction, they were equally likely to make main effect comparisons and pair-wise comparison at first, but shifting to make pair-wise comparisons more by their second and third conclusions. Comparing Figure \ref{fig:bar_all}a and \ref{fig:bar_all}b suggests that there is no significant effect of color mapping on the overall conclusion type or ranking order ($\chi^2 = 6.28$, $p = 0.18$), such that the conclusions people draw follows the same pattern between congruent color-spatial mapping and incongruent color-spatial mapping. Table \ref{color_all} further shows that overall, color grouping does not have an effect on what conclusion categories people draw. In order words, coloring the variable that is not spatially grouped (e.g., bar charts with color grey, white, grey, white) does not make people more likely to draw pair-wise comparisons or overall between comparisons. 

\begin{table}[h]
\renewcommand{\arraystretch}{1.1} \small \centering
\rowcolors{2}{gray!25}{white} 
\renewcommand{\arraystretch}{1.3}
  \caption{Color Overall - should be no difference.}
  \begin{tabular}{llll}
  \newline \\ {\bf Category} & {\bf No Mapping} & {\bf Incongruent} & {\bf Congruent} \\ \hline 
main between & 1.00 & 1.00  & 1.00  \\
 main within & 1.45*  &  $1.39^{.}$ &  2.24*** \\
 pair-wise between & 0.80 & 0.78  &  1.24 \\
 pair-wise within & 0.64*  &  0.85 & 0.82 \\
 interaction between & 0.10*** & 0.42***  & 0.12*** \\
 interaction within & 0.38*** & 0.37***  & $0.65^{.}$  \\
    \end{tabular}
    \label{color_all}
\end{table}



\subsubsection{Effects of Data Relation}
We further examine how additional color grouping affects conclusions draw from charts with varying underlying data relations, as shown in Figure \ref{fig:DataRelationAll}. 

Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with color grouping for each data relations further shows XXXXXX. Table \ref{FirstConclusionOR} shows the odds ratio of participants drawing a specific comparison as their \textit{first} conclusion for each of the three data relations. 

\begin{table}[h]
\renewcommand{\arraystretch}{1.1} \small \centering
  \caption{Color Overall by Data Relation}
  \begin{tabular}{lllll}
  \newline \\ {\bf Data Relation} & {\bf Category} & {\bf No Mapping} & {\bf Incongruent} & {\bf Congruent} \\ \hline 
\multirow{6}{3em}{No Main Effect, Yes Interaction} & \rowcolor{gray!25} main between & 1.00  & 1.00  & 1.00  \\
 & main within & 1.20  &  1.88  &  4.00**  \\
 & \rowcolor{gray!25} pair between & $2.00^{.}$ & 1.66 &  \textbf{5.40***}  \\
 & pair within & \textbf{2.60*}  &  \textbf{3.11**}  &  3.60* \\
 & \rowcolor{gray!25} int. between & 0.00 & 0.44  & 0.00 \\
 & int. within & 1.10  & 1.11  &   2.20 \\ \hline 
 
 \multirow{6}{3em}{One Main Effect, No Interaction} & \rowcolor{blue!15} main between &  1.00 & 1.00  & 1.00  \\
 & main within & \textbf{2.16**}  &  \textbf{2.58**}  & \textbf{4.00**}  \\
 & \rowcolor{blue!15} pair between & 0.83  & $1.83^{.}$  & 1.80  \\
 & pair within & 0.22**  &  1.08  &  0.50 \\
 & \rowcolor{blue!15} int. between & 0.22** &  0.83 & 0.19* \\
 & int. within & $0.44^{.}$ & 0.74  &  1.30 \\ \hline 
 
 \multirow{6}{3em}{Two Main Effects, No Interaction} & \rowcolor{gray!25} main between & 1.00  & \textbf{1.00}  & 1.00 \\
 & main within & \textbf{1.10}  & 0.85  &  \textbf{1.23}  \\
 & \rowcolor{gray!25} pair between & 0.37**  & 0.20***  &  0.23** \\
 & pair within & 0.24***  & 0.20***   &  0.42* \\
 & \rowcolor{gray!25} int. between & 0.06*** & 0.28***  & 0.12*** \\
 & int. within &  0.10*** &  0.05*** & 0.12***  \\
    \end{tabular}
    \label{color_all}
\end{table}

\subsubsection{Interaction between Color, Size, and Spatial Grouping}
We further compare the effect of color grouping for when participants draw conclusions from different data set. More specifically, we compare the odds ratio of participants comparing the two spatially approximate group for when the color grouping is congruent and incongruent with the spatial grouping, across the four possible size grouping discussed in section \ref{1asize}. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{Color and Size}
  \begin{tabular}{lllll}
  \newline \\ {\bf Within} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\ 
  \hline 
 No Color Mapping & 1.00 & 1.00 & 1.00  & 1.00  \\
 Color-Spatial Incongru. & 1.15 & 1.04 & 0.86  &  1.12 \\
 Color-Spatial Congru. & 1.57* & 1.16  & 0.81 &  1.00 \\
 
 \newline 
 \newline \\ {\bf Between} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\ 
  \hline 
 No Color Mapping & 1.00 & 1.00 & 1.00  & 1.00  \\
 Color-Spatial Incongru. & 0.99  & 1.18 & 1.27  &  0.93  \\
 Color-Spatial Congru. &  0.24* &  0.63  & 1.01  & 1.07   \\
 
 \newline \rowcolor{white}
  \newline  \\ {\bf Total} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\
 \hline 
 \rowcolor{gray!25} Within & 2.11** & 1.00 & 0.40*** & 1.70***  \\
 \rowcolor{white} Between & 0.29**  & 0.60 & 1.51***  & 0.35***   \\
 
    \end{tabular}
    \label{sizegrouping_1111}
\end{table}

We see that color grouping doesn't make a big difference in what people would contribute. On the other hand, we see that size mattered a lot + a main effect of spatial grouping. 

Overall - 60\% more likely to use say spatial grouping
This can double or be halved depending on the size grouping.

Color grouping doesn't make much difference. 


%% DISCUSSION %%
\subsection{Discussion}
Overall, for bar graphs with two binary factors (four total bars) with competing groupings of proximity, color, and size, participants were most likely to group and compare marks with similar sizes (e.g., the average of these two large values is larger than of those two small values), followed by comparing spatially proximal marks, followed by groups of the same color.



%%% No color below

%% Bar Visualization Design Space%%
\begin{figure}[th]
 \includegraphics[width=3.4in]{BarDesignSpace.jpg}
 \caption{Design Space for Bar Graph Experiments. Talk about alternating color for each relation. }
 \label{fig:exp1design}
\end{figure}

\begin{figure*}[t]
 \includegraphics[width=17cm]{bar.jpg}
 \caption{Conclusions by Underlying Data Relations details, visualized both by aggregating category (top) and by aggregating rank (bottom) for experiment 1a and 1b, following the spirit of the paper.}
 \label{fig:bar_all}
\end{figure*}


%% EXPERIMENT 1 %%
\section{Experiment 1 Bar Visualizations}
To investigate the effect of spatial, color and size grouping, we selected three combinations of main effects and interactions to cover six of the unique and interesting relations from the eight possibilities as shown in Figure \ref{fig:eightRelationships}, in hopes of balancing potential confound created by data relations and size grouping. We created three data sets with three different underlying relations: one data set with no main effect but an interaction (h), one with one main effect but no interaction (b/c), and one with two main effects but no interaction (a). We used the same two factors (company and region) from the pilot. Each data set is presented as a bar chart either spatially grouped by company or by region, subsequently making the size grouping either congruent or incongruent to the spatial grouping. We also incorporated a color dimension for each chart. Color is either mapped onto region or company, making it either congruent or incongruent with spatial grouping. Congruent color-spatial mapping means the spatially approximate two bars share the same color (e.g., grey, grey, white, white), while incongruent color-spatial mapping means the spatially approximate two bars have different colors (e.g., grey, white, grey, white). Figure \ref{fig:exp1design} maps out the design space. The data sets used to produce each chart were perturbed with some noise to be not entirely uniform. 

\subsection{Data Relation, Spatial and Size Grouping}
We first investigate how spatial and size grouping affect conclusions people draw without considering color grouping, as shown in Figure \ref{fig:exp1design}(a). This experiment follows the same procedure as the pilot experiment. Participants viewed these bar charts and wrote down their top three conclusions. Power analysis based on the pilot effect sizes derived from logistic regression models suggested a target sample of 45 conclusions per category (e.g., main effects, interactions, pair-wise) would give us 80\% power to detect patterns in conclusion frequencies at alpha level of 0.05 \cite{hsieh1998simple}. Because we have no control over the conclusions a given participant would draw from a visualization, we iteratively surveyed and excluded participants on Amazon's Mechanical Turk who gave nonsensical answers or failed attention tests until we have at least 45 conclusions for each bar charts.

%% DESIGN AND PROCEDURE %%
\subsubsection{Summary Statistics on Conclusion Categories}
The conclusions come from 102 unique participants ($M_{age} = 40.02$, $SD_{age} = 9.99$, 40 females), each writing their top three conclusions (in the order of which came to mind first). After excluding the nonsensical conclusions, we ended up with 292 conclusions. As shown in Figure \ref{fig:bar_all}, amongst them, most were conclusions on main effects (47.9\%), followed by pair-wise comparisons (32.2\%), with few interactions (9.59\%), superlatives (7.54\%), and others (2.74\%).

As shown in Table \ref{barRankCategoryORTable}, multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion rankings with conclusion categories suggests that people were most likely to make a main effect comparison first. For those who didn't make a main effect comparison, they were more likely to have made a pair-wise comparison than anything else ($p_{interaction} = 0.002$, $p_{superlative} = 0.001$, $p_{other} < 0.001$). By the second conclusion, people are more likely to make a main effect comparison or a pair-wise comparison than other conclusions, but the likelihood of them making main effect comparison and pair-wise comparison was not significantly different ($p = 0.74$). By the third conclusion, people became more likely to make main effect comparisons again, and similar to what they did for the first conclusion, those who didn't make a main effect comparison more likely made pair-wise comparisons ($p_{interaction} = 0.02$, $p_{superlative} = 0.004$, $p_{other} < 0.001$). More statistical details can be found in the supplementary materials.

More specifically, the prominence of pair-wise comparisons seemed to be largely driven by people more likely making pair-wise comparisons  when the underlying data depicted no main effect but an interaction, as shown in Figure \ref{fig:bar_allSeparatedByRank}. We take a closer look at how underlying data relations could drive the conclusions people make.

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
\renewcommand{\arraystretch}{1.3}
  \caption{How likely did people draw these different types of conclusions compared to a main effect, for each rank. How to interpret the numbers: a value of 0.51 for pair-wise comparison under First Rank means the odds of a participant drawing a pair-wise conclusion is 0.51 that of drawing a main effect conclusion.}
  \begin{tabular}{lrrr}
  \newline \\ {\bf Category} & {\bf First Rank} & {\bf Second Rank} & {\bf Third Rank} \\ \hline 
 main & 1.00 &  1.00 & 1.00 \\ pair-wise & 0.51 & 1.08 & 0.52 \\ interaction & 0.15 & 0.26 & 0.22\\
 superlative & 0.13 & 0.21 & 0.15 \\ others & 0.07 & 0.05 & 0.04 \\
    \end{tabular}
    \label{barRankCategoryORTable}
\end{table}











%% Results %%
\subsubsection{Effect of Underlying Data Relation}
A $\chi^2$ test of independence with Bonferroni adjustment suggests that people more likely made main effect comparisons when they viewed data depicting one main effect and no interactions, or two main effects and no interactions, compared to data depicting an interaction but no main effects ($\chi^2 = 43.69$, $p < 0.001$). Post-hoc comparisons with Bonferroni corrections revealed that they were more likely to make pair-wise comparisons when viewing data depicting an interaction but no main effects ($z = 5.92$, $p < 0.001$). They were marginally less likely to draw interaction comparisons when viewing data depicting two main effects with no interactions compared to the other two ($z = -1.82$, $p = 0.06$). 

As shown in Figure \ref{fig:DataRelationAll}, conclusions varied with rank and underlying data relations. Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with data relations further shows that people take into consideration the underlying data relation as they make comparisons of data. Table \ref{FirstConclusionOR} shows the odds ratio of participants drawing a specific comparison as their \textit{first} conclusion for each of the three data relations. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{How likely did people draw these different types of conclusions as the FIRST CONCLUSION for each data relation type. \cx{consider replace NoMainYesInt header with mini pictures}}
  \begin{tabular}{lrrr}
  \newline \\ {\bf Conclusion} & {\bf No Main Yes Int} & {\bf One Main Only} & {\bf Two Main Only} \\ 
  \hline 
 main between & 1.00 & 1.00 & 1.00 \\
 main within & 3.00 & \textbf{2.28} & \textbf{1.66} \\
 pair-wise between & 2.50 & 0.71 & 0.33 \\
 pair-wise within & \textbf{6.00} & 0.29 & 0.11 \\
 interaction between & <0.01 & 0.14 & 0.11\\
 interaction within & 2.00 & 0.29 & <0.01 \\
    \end{tabular}
    \label{FirstConclusionOR}
\end{table}

For bar charts depicting an interaction but no main effect, the majority of conclusions were pair-wise comparisons. People were the most likely to first make a within-group pair-wise comparison (and specifically, of the left group). Those who didn't make a within-group pair-wise comparison would likely make a within-group main effect comparison or a between-group pair-wise comparison. For their second conclusion, they switch to make either a between-group or a within-group pair-wise comparison of the right group. Very few participants made pair-wise proximity and edge comparisons (~6\%). For those who did, these comparisons were often the second or third conclusion people drew, never the first. We omit these comparisons from the detailed visualization as shown in Figure \ref{fig:exp1aMain0Int1PairwiseDetail}.

For bar charts depicting one main effect and no interaction, the majority of conclusions were main-effect comparisons. People were the most likely to make within-group main comparisons as their first conclusion, as shown in figure \ref{fig:DataRelationAll}. In fact, participants mostly make within-group main effect comparisons for their second and third comparisons as well. Those who didn't make main-effect comparisons mostly made pair-wise between-group comparisons. 

For bar charts depicting two main effects and no interaction, people likely first made a within-group main effect comparison. For their second conclusion, they either switched to make a between-group main effect comparison, or made a pair-wise comparison. Different from those who viewed bar charts depicting one main effect, participants who viewed bar charts depicting two main effects were equally likely to make between-group and within-group pair-wise comparisons. 

A closer look at the specific pair-wise comparisons participants made demonstrates that people tend to start with a between-group pair comparison of the two tallest bars, then switching to a between-group comparison of the two-shortest bars (East B and West B), see Figure \ref{fig:DataRelationAll}.





%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[th]
 \includegraphics[width=17.8cm]{SizeGrouping.jpg}
 \caption{How size grouping change the balance between the within-group and between-group conclusions people drew. Error bar shows standard error. }
 \label{fig:SizeGrouping}
\end{figure*}

\subsubsection{Effect of Size Grouping}
\label{1asize}
As previously mentioned in section \ref{insightFromPilot}, both the underlying data relation (whether there exists main effect/interaction in the data or not) and size grouping could influence the conclusions people draw. 

We sorted the bar charts into four size grouping categories. As shown in the top of Figure \ref{fig:SizeGrouping}, size grouping could be congruent with spatial grouping such that the two similarly large bars are spatially approximate, and the two similarly small bars are spatially approximate. An example of this category is the "one main effect, no interaction" chart that is grouped by company, see Figure \ref{fig:exp1design}. The second category is a variation that arranges the bars in decreasing size. An example of this category is the "two main effects, no interaction" chart that is grouped by region. This decreasing grouping still maintains spatial-size congruency, such that the two larger bars are spatially approximate, and the two smaller bars are spatially approximate. The third category is when size and spatial grouping are incongruent, such that the spatially approximate two bars significantly differ in size. An example of this is the "one main effect, no interaction" chart grouped by region. The fourth category is a variation that is also size-spatial incongruent where the tallest two bars are the furthest away from each other. Examples include the "no main effect, yes interaction" charts. 

Overall, by aggregating size grouping, we see that people tend to draw the within-group conclusions comparing the two spatially separated groups when spatial grouping is congruent with size grouping, as shown in the left most column in the top section of Figure \ref{fig:SizeGrouping}. As the size grouping become more and more incongruent with spatial grouping, people became more likely to draw a balance amount of both within-group and between-group conclusions. This shows a competition between spatial and size grouping, suggesting both are of equal strength and both drive what a viewer would conclude. More specifically, if spatial grouping is the stronger driver, you would expect participants to always make within-group main comparisons. If size-grouping is the stronger driver, you would expect participants to always make between-group main comparisons when the tall and short bars alternate in the chart. We see that this is not the case.

We discuss in depth a scenario where the underlying data is the same but size grouping changes: one congruent with spatial grouping such that the bars with similar height were also spatially placed together, and one incongruent with spatial grouping such that the bars with dissimilar sizes were spatially placed together, as shown in the first and third columns in the Figure \ref{fig:SizeGrouping} left block (the right block is showing the same data as the left block, but arranged in a different way following the spirit of the paper). More specifically, both charts depict one main effect and no interaction, but one is grouped by company on the x-axis and the other is grouped by region. We see that more people made within group main effect and interaction comparison between the two spatially separated group when size-spatial grouping is congruent. There is no difference in the pair-wise comparisons they made. Table \ref{sizegrouping_1111} shows the results of a  multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with size grouping. The likelihoods of participants drawing a particular conclusion under each size grouping are compared. More details can be found in the supplementary materials. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{How likely did people draw these different types of conclusions for each size grouping}
  \begin{tabular}{lllll}
  \newline \\ {\bf Conclusion} & {\bf Congruent} & {\bf Decreasing} & {\bf Incongruent} & {\bf Polarizing} \\ 
  \hline 
 main between & 1.00 & 1.00 & \textbf{1.00} & 1.00*** \\
 main within & \textbf{6.09}** & \textbf{2.00} & 0.89 & 2.04*** \\
 pair-wise between & 1.29 & 0.28*** & 0.64* & 2.58*** \\
 pair-wise within & 1.49 & 0.31** & 0.25*** & \textbf{2.99}*** \\
 interaction between & 0.39 & 0.12*** & 0.26*** & 0.16** \\
 interaction within & 2.09* & 0.09*** & 0.15*** & 1.33\\
    \end{tabular}
    \label{sizegrouping_1111}
\end{table}



\subsubsection{Discussion}
Underlying data relation influences the category of conclusions people make (e.g., main effect or pair-wise comparison), whereas the size grouping influences the comparisons people make (e.g., between or within). When the underlying data depicts one main effect, people likely would first do a main effect comparison between the two spatially grouped levels. When the underlying data depicts two main effects, people alternate between the within-group and the between-group main effect comparisons, first doing a within-group main effect comparison between the two spatially grouped levels, followed by a between-group main effect comparison between the two levels not spatially grouped. When the underlying data depicts no main effect but an interaction, people tend to make within group pair-wise comparisons. Size-grouping interacts with the effect of underlying data relations such that congruent size-spatial grouping leads to more main effect comparisons (more specifically, within-group ones) and more within-group interaction comparisons, and incongruent size-spatial grouping leads to more pair-wise comparisons.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{exp1color}

==> BackupTex/backup_exp1_only <==
\subsubsection{Effect of Underlying Data Relation}
\label{dataRelationSection}
A $\chi^2$ test of independence with Bonferroni adjustment suggests that people more likely made main effect comparisons when they viewed data depicting one main effect and no interactions, or two main effects and no interactions, compared to data depicting an interaction but no main effects ($\chi^2 = 43.69$, $p < 0.001$). Post-hoc comparisons with Bonferroni corrections revealed that they were more likely to make pair-wise comparisons when viewing data depicting an interaction but no main effects ($z = 5.92$, $p < 0.001$). They were marginally less likely to draw interaction comparisons when viewing data depicting two main effects with no interactions compared to the other two ($z = -1.82$, $p = 0.06$). 

As shown in Figure \ref{fig:DataRelationAll}, conclusions varied with rank and underlying data relations. Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with data relations further shows that people take into consideration the underlying data relation as they make comparisons of data. Table \ref{FirstConclusionOR} shows the odds ratio of participants drawing a specific comparison as their \textit{first} conclusion for each of the three data relations. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{How likely did people draw these different types of conclusions as the FIRST CONCLUSION for each data relation type. \cx{consider replace NoMainYesInt header with mini pictures}}
  \begin{tabular}{lrrr}
  \newline \\ {\bf Conclusion} & {\bf No Main Yes Int} & {\bf One Main Only} & {\bf Two Main Only} \\ 
  \hline 
 main between & 1.00 & 1.00 & 1.00 \\
 main within & 3.00 & \textbf{2.28} & \textbf{1.66} \\
 pair-wise between & 2.50 & 0.71 & 0.33 \\
 pair-wise within & \textbf{6.00} & 0.29 & 0.11 \\
 interaction between & <0.01 & 0.14 & 0.11\\
 interaction within & 2.00 & 0.29 & <0.01 \\
    \end{tabular}
    \label{FirstConclusionOR}
\end{table}

For bar charts depicting an interaction but no main effect, the majority of conclusions were pair-wise comparisons. People were the most likely to first make a within-group pair-wise comparison (and specifically, of the left group). Those who didn't make a within-group pair-wise comparison would likely make a within-group main effect comparison or a between-group pair-wise comparison. For their second conclusion, they switch to make either a between-group or a within-group pair-wise comparison of the right group. Very few participants made pair-wise proximity and edge comparisons (~6\%). For those who did, these comparisons were often the second or third conclusion people drew, never the first. We omit these comparisons from the detailed visualization as shown in Figure \ref{fig:exp1aMain0Int1PairwiseDetail}.

For bar charts depicting one main effect and no interaction, the majority of conclusions were main-effect comparisons. People were the most likely to make within-group main comparisons as their first conclusion, as shown in figure \ref{fig:DataRelationAll}. In fact, participants mostly make within-group main effect comparisons for their second and third comparisons as well. Those who didn't make main-effect comparisons mostly made pair-wise between-group comparisons. 

For bar charts depicting two main effects and no interaction, people likely first made a within-group main effect comparison. For their second conclusion, they either switched to make a between-group main effect comparison, or made a pair-wise comparison. Different from those who viewed bar charts depicting one main effect, participants who viewed bar charts depicting two main effects were equally likely to make between-group and within-group pair-wise comparisons. 

A closer look at the specific pair-wise comparisons participants made demonstrates that people tend to start with a between-group pair comparison of the two tallest bars, then switching to a between-group comparison of the two-shortest bars (East B and West B), see Figure \ref{fig:DataRelationAll}.





%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[th]
 \includegraphics[width=17.8cm]{SizeGrouping.jpg}
 \caption{How size grouping change the balance between the within-group and between-group conclusions people drew. Error bar shows standard error. }
 \label{fig:SizeGrouping}
\end{figure*}

\subsubsection{Effect of Size Grouping}
\label{1asize}
As previously mentioned in section \ref{insightFromPilot}, both the underlying data relation (whether there exists main effect/interaction in the data or not) and size grouping could influence the conclusions people draw. 

We sorted the bar charts into four size grouping categories. As shown in the top of Figure \ref{fig:SizeGrouping}, size grouping could be congruent with spatial grouping such that the two similarly large bars are spatially approximate, and the two similarly small bars are spatially approximate. An example of this category is the "one main effect, no interaction" chart that is grouped by company, see Figure \ref{fig:exp1design}. The second category is a variation that arranges the bars in decreasing size. An example of this category is the "two main effects, no interaction" chart that is grouped by region. This decreasing grouping still maintains spatial-size congruency, such that the two larger bars are spatially approximate, and the two smaller bars are spatially approximate. The third category is when size and spatial grouping are incongruent, such that the spatially approximate two bars significantly differ in size. An example of this is the "one main effect, no interaction" chart grouped by region. The fourth category is a variation that is also size-spatial incongruent where the tallest two bars are the furthest away from each other. Examples include the "no main effect, yes interaction" charts. 

Overall, by aggregating size grouping, we see that people tend to draw the within-group conclusions comparing the two spatially separated groups when spatial grouping is congruent with size grouping, as shown in the left most column in the top section of Figure \ref{fig:SizeGrouping}. As the size grouping become more and more incongruent with spatial grouping, people became more likely to draw a balance amount of both within-group and between-group conclusions. This shows a competition between spatial and size grouping, suggesting both are of equal strength and both drive what a viewer would conclude. More specifically, if spatial grouping is the stronger driver, you would expect participants to always make within-group main comparisons. If size-grouping is the stronger driver, you would expect participants to always make between-group main comparisons when the tall and short bars alternate in the chart. We see that this is not the case.

We discuss in depth a scenario where the underlying data is the same but size grouping changes: one congruent with spatial grouping such that the bars with similar height were also spatially placed together, and one incongruent with spatial grouping such that the bars with dissimilar sizes were spatially placed together, as shown in the first and third columns in the Figure \ref{fig:SizeGrouping} left block (the right block is showing the same data as the left block, but arranged in a different way following the spirit of the paper). More specifically, both charts depict one main effect and no interaction, but one is grouped by company on the x-axis and the other is grouped by region. We see that more people made within group main effect and interaction comparison between the two spatially separated group when size-spatial grouping is congruent. There is no difference in the pair-wise comparisons they made. Table \ref{sizegrouping_1111} shows the results of a  multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with size grouping. The likelihoods of participants drawing a particular conclusion under each size grouping are compared. More details can be found in the supplementary materials. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{How likely did people draw these different types of conclusions for each size grouping}
  \begin{tabular}{lllll}
  \newline \\ {\bf Conclusion} & {\bf Congruent} & {\bf Decreasing} & {\bf Incongruent} & {\bf Polarizing} \\ 
  \hline 
 main between & 1.00 & 1.00 & \textbf{1.00} & 1.00*** \\
 main within & \textbf{6.09}** & \textbf{2.00} & 0.89 & 2.04*** \\
 pair-wise between & 1.29 & 0.28*** & 0.64* & 2.58*** \\
 pair-wise within & 1.49 & 0.31** & 0.25*** & \textbf{2.99}*** \\
 interaction between & 0.39 & 0.12*** & 0.26*** & 0.16** \\
 interaction within & 2.09* & 0.09*** & 0.15*** & 1.33\\
    \end{tabular}
    \label{sizegrouping_1111}
\end{table}



\subsubsection{Discussion}
Underlying data relation influences the category of conclusions people make (e.g., main effect or pair-wise comparison), whereas the size grouping influences the comparisons people make (e.g., between or within). When the underlying data depicts one main effect, people likely would first do a main effect comparison between the two spatially grouped levels. When the underlying data depicts two main effects, people alternate between the within-group and the between-group main effect comparisons, first doing a within-group main effect comparison between the two spatially grouped levels, followed by a between-group main effect comparison between the two levels not spatially grouped. When the underlying data depicts no main effect but an interaction, people tend to make within group pair-wise comparisons. Size-grouping interacts with the effect of underlying data relations such that congruent size-spatial grouping leads to more main effect comparisons (more specifically, within-group ones) and more within-group interaction comparisons, and incongruent size-spatial grouping leads to more pair-wise comparisons.

==> BackupTex/backup_exp1color.tex <==
\subsection{Additional Consideration of Color Grouping}
We observed a competition between spatial and size grouping in Experiment 1a. We further investigate how color grouping interacts with spatial and size grouping by 

\subsubsection{Summary Statistics on Conclusion Categories}
The conclusions come from 210 unique participants ($M_{age}$ = 40.91, $SD_{age}$ = 9.95, 85 females). After excluding the nonsensical conclusions, we ended up with 605 conclusions. Similar to Experiment 1a, most conclusions were main effects(44.1\%), followed by pair-wise comparisons (31.7\%), with few interactions (12.7\%), superlatives (6.94\%), and others (4.47\%). 

%\As shown in Figure \ref{fig:bar_all}b, participants who viewed the bar charts with the additional color mapping seem to follow the same pattern as those that viewed the bar charts without the color mapping. They were more likely to make main effect comparisons for data depicting one main effect and no interaction, and data depicting two main effects and no interaction. When they viewed data depicting no main effect but an interaction, they were equally likely to make main effect comparisons and pair-wise comparison at first, but shifting to make pair-wise comparisons more by their second and third conclusions. Comparing Figure \ref{fig:bar_all}a and \ref{fig:bar_all}b suggests that there is no significant effect of color mapping on the overall conclusion type or ranking order ($\chi^2 = 6.28$, $p = 0.18$), such that the conclusions people draw follows the same pattern between congruent color-spatial mapping and incongruent color-spatial mapping. Table \ref{color_all} further shows that overall, color grouping does not have an effect on what conclusion categories people draw. In order words, coloring the variable that is not spatially grouped (e.g., bar charts with color grey, white, grey, white) does not make people more likely to draw pair-wise comparisons or overall between comparisons. 





\subsubsection{Effects of Data Relation}
We further examine how additional color grouping affects conclusions draw from charts with varying underlying data relations, as shown in Figure \ref{fig:DataRelationAll}. 

Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with color grouping for each data relations further shows XXXXXX. Table \ref{FirstConclusionOR} shows the odds ratio of participants drawing a specific comparison as their \textit{first} conclusion for each of the three data relations. 






%% DISCUSSION %%
\subsection{Discussion}
Overall, for bar graphs with two binary factors (four total bars) with competing groupings of proximity, color, and size, participants were most likely to group and compare marks with similar sizes (e.g., the average of these two large values is larger than of those two small values), followed by comparing spatially proximal marks, followed by groups of the same color.


==> BackupTex/backup_future.tex <==
%% DISCUSSION %%
\section{General Conclusion}


Size, spatial, color, then shape overall. 

Mostly compare main effect, but certain size grouping makes ppl want to compare pair-wise.

Interaction is hard. Can be enhanced by color and size grouping. 

!! We mapped out the conclusion space for simple bar charts and scatterplots. One future direction is to map conclusion space to different vis. and action. 


%% LIMITATIONS AND FUTURE DIRECTIONS %%
\section{Limitations and Future Directions}
\label{limitation}

\textbf{Visual Routine} 
% discussion of potential confound of left bar always being the tallest 
In the bar charts tested so far, we noticed that participants tend to draw conclusions starting from the left of the visualization. In bar charts depicting no main effect but an interaction ( bars in order of tall, short, short, tall), the majority of the people made pair-wise comparisons with the two bars on the left. In bar charts where size and spatial groupings were incongruent (bars in order of tall, short, tall, short), participants drew pair-wise comparisons between the tallest two bars, one of which being the left-most. We have yet to tease apart whether this was driven by a tendency to focus on the tallest bars or to start from the left of the visualization. Experiment 1b investigate this position-size confound to further dissect how spatial arrangement and size grouping interacts to influence the conclusions people draw.

Future: Position-Size Investigation

\subsection{Other Visualization Components to Examine}
words
\label
Kossyn \cite{kosslyn2006graph} decomposed graphs into 5 components (background, caption, framework, labels and content). All five consists of testable visual elements that could influence the type of visual comparisons/chunking we do and the sentence we generate.
Background: color, 
Captions:
Framework: axes
Content: point, lines, bars
Labels: variable names, title, axes, legend,

+ also other encoding chanels to rank (not in accuracy, but in saliency!)

\subsection{Future investigation for scatterplots on color and shape}
peopel more likely comapred the two groups with different shape of the same color, such as comparing fuel economy of striaght engine for auto and manual transmision, when transmission is encoded by shape and engine by color. This could suggest that the higher ranked, more salient grouping cues like color in a color and shape competition, would be compared on a higher/more aggregated level, while less salient grouping cues, like shape, would be compared on a more granular level.
Future investigation should see if this pyramidal structure of comparison happens with other things. For example, we know spatial proximity is more salient than color, would people select two spatially approximate thing 

\subsection{Visualization Type Dependent Ranking of Grouping Cues}
While we found spatial > size > color for bars, and color > shape for scatter, these rankings could be visualization type dependent, such that color could be more salient than size in scatter plots. Mention Danielle's paper, we know the discriminability of color changes with size, future people can expand this ranking system to more systematically test various size and color pairing. E.g., These color pairs vs. these size, color is better. But these color pairs vs. these size that's very similiar, size is better. Or do the same with spatial grouping.  

% future
extend to complex data. 
can we develope metrics to preidct what people will say when they look at a vis, and use that to measure how difficult graphs are to comprehend.

% limitation
We didn't do any understanding stuff
Here is some related background: 
Technique for Measuring Comprehension of visualizations: evaluate whether people understand it or not. There are multiple teests of graph literacy or interpretation. Standard practice is having eperts in a field to produce a test \cite{royer1981theory}. Covering the range of forms for
statistical graphics requires a large corpus of questions \cite{wainer1980test}. Recent researchers have developed an algorithmic method to generate queries to measure comprehension for statistical graphs \cite{livingston2019query}. They introduced the idea of visualization as analogy to sentences. There exist an original source visualization, and paraphrase visualizations that communicates a gist of the source visualization. Participants would determine whether the information shown in the paraphrased visualization was stated or not stated in the source graph.

% Future %
\subsection{future}
People can model stuff. Like these folks already did. 
1.Modeling a Graph Viewer’s Effort in Recognizing Messages Conveyed by Grouped Bar Charts, Richard Burns
2. Automatically Recognizing Intended Messages in Grouped Bar Charts (Richard Burns1, Sandra Carberry1, Stephanie Elzer2, and Daniel Chester)

Other comparision components?
3. facet? How would facet influence conclusions? People might get confused by facet (think the two x-axis are one axis). How can we leverage it to elicit comparisons? 
4. numerosity (1000 of A, 10 of B, what do people compare) and spatial separability. What do people compare? 


interesting: heuristic erros where they look at the left most bar and made more general claim than they should "East is bigger (when it's not actually" - see coding page for heuristic error. Cite Elsie's thing about heuristics


\textbf{Other usages for sentence generation investigation and modeling} text visualization, help blind people, natural language based visualization recommendation systems
Cite: 
https://www.mitpressjournals.org/doi/pdf/10.1162/COLI_a_00091 (Summarizing Information Graphics Textually)

https://www.aclweb.org/anthology/W11-2703.pdf
(A Corpus of Human-written Summaries of Line Graphs)

%% SUMMARY%%
\section{Design Guidelines}
some guidelines
something about recommendation systems (see https://medium.com/multiple-views-visualization-research-explained/insight-machines-the-past-present-and-future-of-visualization-recommendation-2185c33a09aa)

Future People can use this to build stuff! 

I also plan to develop actionable design guidelines that mitigate biases and support critical thinking with data. I will develop visualization systems that help people make more effective data-driven decisions. For example, since visualization design can afford different thinking patterns with data, I plan to use crowd-sourcing in order to create a database of possible comparisons, inferences, and decisions people draw from data and develop a general framework that can predict what a person would conclude upon seeing a visualization. From it, I can develop an intelligent system that adjusts the visual presentation of data to avoid misguided interpretations and make data more accessible.

% having more potential visual groups is difficult. 
% Having more variety of visual groups channels is difficult - color, and shape, and size, etc (visual searh and stimulus similarity, duncan and humphreys

==> Exp3.tex <==
\section{Experiment 3}

% Hypothesis 8: In group comparisons, once people make a near group comparison, they will be less likely to make a far group comparison, and vice versa. This effect will be more pronounced when more grouping cues (e.g., color, size, and spatial proximity) are congruent. 
Experiment 3 allowed us to evaluate Hypothesis 8, concerning whether grouping cues can drive one group comparison so strongly that the other group comparison becomes difficult to detect. We used the same six charts depicting the same three data sets, except that the bars were recolored such that the two spatially proximate bars had the same color \andrew{Reference the figure for Experiment 3 stimuli here.}. This made the spatial proximity grouping cue and the color grouping congruent, which should increase the salience of near groups. Using these charts, we examined whether overly strong grouping cues would make people become less likely to compare the groups without those cues. 

\andrew{I don't see anything in the Exp results that addresses Hypothesis 8. If you wanted to address Hypothesis 8, you would presumably look at something like: Are participants less likely to make one group comparison as their third conclusion if they're already made the other group comparison as one of their earlier conclusions?}

\andrew {Given that Exp 3 doesn't address Hypothesis 8. I'm not sure what this experiment contributes to the paper. I would suggest the following:
1) Remove Exp 3.
2) To address the question of whether color cues contribute to grouping, compare the near/far grouping rates in Exp 1 vs. Exp 2.
3) If you want to test Hypothesis 8, conduct something like the analysis I suggested above, but for Exp 2. Alternatively (since that might be a lot of extra work and we're short on time), remove Hypothesis 8 and change it to a prediction that we can bring up in the discussion section. Although it's a little strange to have a prediction that could be tested in the data we already have.}

%% Experiment 2 Pair Comparisons %%
\begin{figure*}[h]
 \includegraphics[width=\linewidth]{Figure/exp3results.jpg}
 \caption{Overall distribution of Exp 3 results}
 \label{exp3results}
\end{figure*}

\subsection{Participants}

We collected sentence conclusions from 102 unique participants ($M_{age} = 39.87$, $SD_{age} = 9.89$, 40 females). Every participant wrote three conclusions (in the order of which came to mind first). After excluding the nonsensical conclusions (7.6\%), we ended up with 316 conclusions total. \andrew {As in Exp 2, I'm curious if you used the same attention criteria as in Exp 1.}

\subsection{Results Overview}

As shown in Figure \ref{exp3results}, for the first conclusion, participants made more group comparisons (46.08\%), followed by pair comparisons (27.45\%), both significantly more often than the other comparison types (${\chi}^2$ = 85.41, p < 0.001). For the second conclusion, participants made more pair comparisons (41.58\%), followed by group comparisons (29.70\%), and both were significantly more frequent than the other comparisons types (${\chi}^2$ = 72.05, p < 0.001). For the third conclusion, participants again made the more group comparisons (44.94\%), followed by pair comparisons (26.97\%), all more often than the other comparison types (${\chi}^2$ = 70.44, $p_{group} < 0.001$, $p_{pair} = 0.054$).

We replicated the finding from Experiment 1 that participants were more likely to do group comparisons as their first comparison and shifted to doing pair comparison as the second comparison. We also replicated the finding that most of the pair comparisons were near (39.36\%) and far (48.94\%) pair comparisons, and very few were center (9.57\%) and edge (2.13\%) comparisons (${\chi}^2$ = 57.92, p < 0.001). We also observed a consistent, low frequency of superlative comparisons (6.86\% as first conclusions, 7.92\% as second conclusions, 7.87\% as third conclusions). \andrew{Just as in Exp 1, we see more far pair comparisons than near pair comparisons. This is weird. I would have predicted way more near comparisons than far comparisons given that the near pairs also match in color.}

\subsection{Hypothesis 8: Grouping Cues and Group Comparisons}

We again counted the number of times participants conducted a near or a far group comparison and found that 34.2\% of them were far comparisons and 65.8\% were near comparisons. Chi-square analysis comparing the frequencies of participants conducting a near versus far comparison between Experiment 2 and Experiment 3 suggests that there is no significant difference in how frequently people made near and far comparisons between the two different coloring schemes (${\chi}^2$ = 2.20, p = 0.14). This means the combined grouping cue of spatial proximity and color was not so strong that it locks people into only comparing near groups. Alternatively, this could suggest that coloring bars that are spatially proximate to each the same does not make spatially proximate group more salient than they already are. \andrew{I would say, "Alternatively, this might suggest that bar colors have little effect on which bars get grouped together." This idea could be tested by looking at the frequency of near vs. far group comparisons in Exp 1. If it's the same across all three experiments, then we can conclude that color doesn't really affect grouping for these stimuli.} Figure \ref{exp23mainGroup_colorSpace}, which compares the frequency of near and far group comparisons in Experiment 2 and Experiment 3, further illustrates that color did not have a strong impact on what groups people formed.

==> Old_Text/Bleh.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Hypothesis Motivaton %
\section{Research Questions and Study Overview}
% Through two crowdsourced experiments, we varied the proximity, color, and shape grouping of data values in bar charts and scatterplots, to create a preliminary model that predicts what comparisons an average viewer would likely produce for a given visualization. Participants viewed charts and typed sentences describing the comparisons they made. These sentences were then qualitatively coded by two independent coders. We document the sequence in which these sentences are produced and map them onto a common set of comparisons in a visualization. With refinement and tests for generalizability, this model could produce firm guidelines on how to design visualizations that effectively communicate an intended pattern in data.

Our stimuli are inspired by the types of simple bar charts found in media and scientific journals. In Experiment 1, participants viewed bar charts with two binary factors (four total bars) with competing groupings of proximity, color, and size. To preview our results, they were the most likely to group and compare spatially proximal marks, followed by comparing marks with similar sizes (e.g., the average of these two large values is larger than of those two small values), followed by groups of the same color. In Experiment 2, participants viewed scatterplots with two binary factors (four clusters), with competing groupings across color and shape. Participants were more likely to compare groups encoded with different colors, before moving on to comparing across shape differences. 

% reference the appropriate sections in RW in each hypothesis so people know how and why we hypothesized that way 
\begin{enumerate}
% this is item 1a
  \item Forest before trees: People would group and compare main effect before they compare individual bars (pair-wise)/do higher order comparisons (interactions) - this is mainly investigation of order things are done. The result that people don't often see interactions goes here. <all data - start with simple analysis and then dig deeper>. Categorize main effect and double-pair-wise separately. We are sure that main happens before pair, but not sure about double-pair-wise. Because double pair-wise requires more comparisons, but main -effect rquires doing an average. Which is easier and more intuitive for people to do? We will find out :D
 % this is item 1b
  \item above, but about frequency
  
  \item How are they grouping and comparing main effects? Option 1 is that they grouped and compared averages. Option 2 is that they grouped, and then created some mental representation of the structure of the group, and then compared that structure to the other group, think structural mapping where attention is drawn to commonalities. This is about taking a deeper dive into the main effects. *Note that this could also apply to interactions. <all data>
  
  % closer look at subset
  \item Only look at the pure main effect (not double pair-wise), and see for the color 1010 sets to see if people like to group spatially more or by color more. 
  % closer look at subset
  \itme Compare Size and Spatial only look at the color 1111 ones where size is incongruent with spatial - look at pure main, double-pair-wise separately? What counts as space wins? The same cues that cause you to group 2 bars together also makes you want to compare those 2 bars if you didn't group them together.
 
\end{enumerate}



\begin{table*}[h]
\centering
\rowcolors{2}{gray!25}{white}
    \scriptsize
    \caption{Examples of conclusions, coded expressions, and categories}. 
    \begin{tabular}{p{1.5cm}p{7.65cm}lll}
   \textbf{Example} & \textbf{Sentence Conclusions} & \textbf{Expression} & \textbf{Category} & \textbf{Comparison} \\ 
   \hline
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/main_distal.jpg}}
    & A has more sales than B. & $A > B$ & Main & Distal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/main_proximal.jpg}}
    & East is worse than West. & $East < West$ & Main & Proximal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/pair_distal.jpg}}
    & A does much better in the West as opposed to the East. & $West_A > East_A$ & Pair-wise & Distal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/pair_proximal.jpg}}
    & A's West region generates more revenue than that of B. & $West_A > West_B$ & Pair-wise & Proximal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/pair_edge.jpg}}
    & A's West region has higher revenue than B's East region. & $West_A > East_B$ & Pair-wise & Edge \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/pair_middle.jpg}}
    & B's West region has higher revenue than A's East region. & $West_B > East_A$ & Pair-wise & Middle \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/int_distal.jpg}}
    & A shows more difference in revenue between the two regions than B. & $|West_A - East_A| > |West_B - East_B|$ & Interaction & Distal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/int_proximal.jpg}}
    & West's profitability fluctuates more than East. & $|West_A - West_B| > |East_A - East_B|$ & Interaction & Proximal \\ 
    \parbox[c]{1em}{\includegraphics[height = 1.3cm]{Figure/superlative.jpg}}
    & Company A West is the best. & $max(4) = West_A$ & Superlative &  \\
    % & The two companies work in the same divisions &  & Others &   \\ 
\hline
\end{tabular}
\label{pilot_equation}
\end{table*}

==> Old_Text/abstract_OLD.tex <==
Reading a visualization is like reading a paragraph. Each sentence is a comparison: the mean of these is higher than those, this difference is smaller than that, this trend is decreasing. What determines which comparisons are made first? The viewer's goal and expertise influence which comparisons are made, but the way that values are visually grouped together within the graph's design also influences those comparisons. 

Research from cognitive psychology suggests that comparisons involve two or three steps: 1) divide the visualization into a set of units, which might include a single bar in a bar chart or a set of bars that have been grouped together; 2) select two of these units and compare them, for example determining that one pair of is longer than another; 3) sometimes, perform a second-order comparison, for example determining that the difference between one pair of bars is greater than the difference between another pair of bars. Based on this view, we create a visual comparison taxonomy that allows us to develop and test a sequence of hypotheses about which comparisons people are more likely to make when viewing a visualization. We find that people tend to compare two groups before comparing two individual units, and that second-order comparisons are rare. Furthermore, we find that visual cues like spatial proximity and can influence which elements are grouped together and selected for comparison. 

Specifically, participants are more likely to group spatially proximal marks, rather than grouping marks of the same color. In contrast, they are equally likely to select and compare either proximal or same-color marks. Because color and spatial cues are easily manipulable by visualization designers, this investigation, along with our comparison taxonomy, can help generate concrete design guidelines to create visualizations that best afford a specific type of comparison. 

% With refinement and tests for generalizability, this model could produce firm guidelines on how to design visualizations that effectively communicate an intended pattern in data.

% Visual cues, such as spatial proximity and color, can influence what people group and select for comparison. We examine how viewer comparisons could be influenced by such cues. As color and spatial cues are easily manipulable by visualization designers, this investigation can help generate concrete design guidelines to create visualizations that best afford a specific type of comparison. This is a critical investigation because once people group the wrong thing, they can get stuck with it and become unable to group and select other things. For simple bar charts, we find that participants are more likely to group and compare spatially proximal marks, rather than comapring marks of the same color. With refinement and tests for generalizability, this model could produce firm guidelines on how to design visualizations that effectively communicate an intended pattern in data.

% We also examine how comparisons can be influenced by visual cues in the visualization, which designers have control over. We specifically examined how the prioritization of comparisons in bar charts are influenced by proximity and color grouping of the visual marks. Using these data, we create simple models to predict comparison priority. For simple bar charts, participants were more likely to group and compare spatially proximal marks, than to compare marks of the same color. With refinement and tests for generalizability, this model could produce firm guidelines on how to design visualizations that effectively communicate an intended pattern in data.

% The core claim is that comparisons tend to involve the following three mechanisms: 1) group the chart into units of interest, for example a pair of bars might be grouped together; 2) compare two units, for example determining that one pair of bars is longer than another; 3) sometimes, perform a second-order comparison, where the results of two previous comparisons are compared. The resulting taxonomy allows us to develop and test a sequence of hypotheses about which comparisons people are more likely to make when viewing a visualization. We found that people tend compare two groups before comparing two individual unites, and that second-order comparisons are rare. 

==> Old_Text/exp1.tex <==
\begin{figure*}[h]
 \includegraphics[width=17.8cm]{Figure/bar.pdf}
 \caption{Conclusions by underlying data relations. Each row section represents the order in which the sentence conclusion was made. Orange color shows distal-group comparisons, purple proximal, and grey others. Each grid box of five bars represents the percentage of participant responses for that fixed number of trials. 
 %Because we cannot control to have an equal number of comparisons made for each category, the bar length presents the percentage of conclusions out of the total number of conclusions per grid box (each grid box adds up to 100\%).
 }
 \label{fig:bar_all}
\end{figure*}


%% EXPERIMENT 1 %%
\section{Experiment 1: Bar Visualizations}

Exp1. Spatial vs. Size
One main, no int. color = 1111
Either grouped by AB or EW.

AB: 4411
EW = 4141

Part 1- EW, compare the likelihood of people grouping by size or space. Space wins. 

Exp2. 
One main, no int. Add color, color = 1010
EW = 4141. 
Add color, show that space still wins. Color has minor effect (some small effect, quantify it)

Exp 3.
One main, no int. Add color, color = 1010
Swap grouping order, AB = 4411
space still wins. but people don't do main comparisons anymore, they do pair-wised comparison, the color shifts their attention to look at a portion of the chart and mentions more interactions.

Exp 4. 
One main, no int. No color = 1111
group by AB.
Take color away from Exp 3.
Spatial group is congruent with size. Show that no one compares pairs anymore, but interestingly people are grouping East and West together to compare main more. 

Conclusion:
space wins.
color doesn't help encourage main effect comparisons - they encourage pair-wise comparisons. 

group the stuff with similar sizes together if you want people to focus on that. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bar Visualization Conclusion}
In general, viewers are the most likely to make main effect comparisons. They made pair-wise comparisons more readily when the underlying data is depicting an interaction but no main effect, or when the size-spatial grouping is incongruent and polarizing (these patterns tend to co-occur, see Figure \ref{fig:eightRelationships}(e). Viewers rarely generated interaction comparisons, even when the underlying data was showing only an interaction with no main effects. When viewers saw this type of charts, they made pair-wise comparisons between spatially adjacent data values.
Surprisingly, varying color mapping in bar visualizations had only a small impact on what comparisons a viewer would make. There was one exception, where color influenced which pair-wise comparison a viewer would make when the data depicted an interaction but no main effect, such that incongruent color-spatial arrangements increased the likelihood of viewers making proximal pair-wise comparisons. On the other hand, size-spatial grouping have a much bigger impact on guiding viewer conclusions. Overall, viewers are approximately 31\% more likely to generate sentence conclusions comparing spatially proximate data values than spatially separated ones, and this tendency can be doubled or halved depending on the size-spatial grouping. 



==> Old_Text/exp1_old.tex <==
\begin{figure*}[h]
 \includegraphics[width=17.8cm]{Figure/bar.pdf}
 \caption{Conclusions by underlying data relations. Each row section represents the order in which the sentence conclusion was made. Orange color shows distal-group comparisons, purple proximal, and grey others. Each grid box of five bars represents the percentage of participant responses for that fixed number of trials. 
 %Because we cannot control to have an equal number of comparisons made for each category, the bar length presents the percentage of conclusions out of the total number of conclusions per grid box (each grid box adds up to 100\%).
 }
 \label{fig:bar_all}
\end{figure*}


%% EXPERIMENT 1 %%
\section{Experiment 1: Bar Visualizations}
To investigate the effect of spatial, color, and size groupings on comparisons, we chose a set of data values and arrangements that minimized potential confounds created by data relations and size grouping. To cover blue subset of the relationships from the eight possibilities shown in Figure \ref{fig:eightRelationships}, we selected three combinations of main effects and interactions (the three top-level columns of Figure \ref{fig:exp1design}). These three datasets have three different underlying relations: one dataset with no main effect but an interaction as in (e), one with one main effect but no interaction as in (b) or (c), and one with two main effects but no interaction as in (d). The datasets used to produce each chart were perturbed with noise (+/- 10\% vertical length) so that no two values were identical. This created trivial interactions even in the no interaction charts; see Figure \ref{fig:exp1design}. Note that (f), (g), and (h) were not selected for examination in the experiment because they are visually similar to (d), (c), and (b), especially after perturbing each with noise.

We used the same two factors (company and region) from the pilot. Each dataset was presented as a bar chart either grouped spatially by company or by region, subsequently making the size grouping either congruent or incongruent to the spatial grouping. We also incorporated color grouping for each chart. Color was either mapped onto region or company, making it either congruent or incongruent with spatial grouping. Congruent color-spatial mapping means the spatially proximate two bars share the same color (e.g., grey, grey, white, white), while incongruent color-spatial mapping means the spatially proximate two bars have different colors (e.g., grey, white, grey, white). Figure \ref{fig:exp1design} maps this design space.

This experiment followed the same procedure as the pilot. Participants viewed these bar charts and wrote down their top three conclusions. A power analysis based on the pilot effect sizes derived from logistic regression models suggested a target sample of 45 conclusions per chart would give 80\% power to detect patterns in conclusion frequencies at alpha level of 0.05 \cite{hsieh1998simple}. Because we have no control over the conclusions a given participant would draw from a visualization, we iteratively surveyed and excluded participants on Amazon's Mechanical Turk who gave nonsensical answers or failed attention tests until we had at least 45 conclusions for each bar chart.









%% Results %%
\subsection{Sentence Conclusion Overview}
We collected sentence conclusions from 312 unique participants ($M_{age} = 40.62$, $SD_{age} = 9.95$, 125 females), each writing their top three conclusions (in the order of which came to mind first). After excluding the nonsensical conclusions (4.2\%), we ended up with 897 conclusions total. As shown in Figure \ref{fig:bar_all} annotation 1, most were conclusions on main effects (45.4\%), followed by pair-wise comparisons (31.9\%), with few interactions (11.7\%), superlatives (7.1\%), and others (3.9\%). More specifically, the prominence of pair-wise comparisons seemed to be largely driven by people more likely making pair-wise comparisons when the underlying data depicted no main effect but an interaction, see Figure \ref{fig:bar_all} annotation 2 (more details discussed in Section \ref{dataRelationSection}). 

% color doesn't matter to conclusion frequency
As shown in Figure \ref{fig:bar_all} annotation 3a+b, participants who viewed the bar charts with the additional color mapping seemed to follow the same pattern as those that viewed the bar charts without the color mapping. There was no significant effect of color mapping on the overall conclusion type or ranking order ($\chi^2 = 6.28$, $p = 0.18$) \cite{ripley2016package}, which suggested that color grouping did not have a significant effect on what conclusion categories people drew. %The conclusions people drew followed the same pattern between no color mapping, congruent color-spatial mapping, and incongruent color-spatial mapping. %For example, coloring the variable that is not spatially grouped (e.g., bar charts with color grey, white, grey, white) does not make people more likely to draw pair-wise comparisons or overall distal comparisons. 
Table \ref{category_color} shows the odds ratio of participants writing sentence conclusions in each category (e.g., main effects) for each color mapping, using distal-group main effect conclusions as reference. Each number shows the percentage likelihood a viewer would make a specific category of sentence conclusion compared to making a distal-group main effect comparison for a specific color mapping. For example, for the no color mapping condition (first column), participants were 1.45 times more likely to make a proximal-group main effect conclusion compared to a distal-group main effect (one asterisk represents p < 0.05, two asterisks represents p < 0.01, three asterisks represents p < 0.001, and a dot represents 0.05 < p < 0.09).

\begin{table}[b]
\renewcommand{\arraystretch}{0.9} \small \centering
\rowcolors{2}{gray!25}{white} 
  \caption{Bar Odds Ratio of Comparison Category by Color Mapping
  %Comparing the likelihood of participants producing sentence conclusions in each category for the three color mapping conditions. Color grouping does not significantly influence the frequency of sentence conclusion in each category.
  }
  \begin{tabular}{llll}
  \newline \\ {\bf Category} & {\bf No Mapping} & {\bf Incongruent} & {\bf Congruent} \\ \hline 
main distal & 1.00 & 1.00  & 1.00  \\
 main proximal & \textbf{1.45}*  &  \textbf{1.39}$^{\bullet}$ &  \textbf{2.24}*** \\
 pair-wise distal & 0.80 & 0.78  &  1.24 \\
 pair-wise proximal & 0.64*  &  0.85 & 0.82 \\
 interaction distal & 0.10*** & 0.42***  & 0.12*** \\
 interaction proximal & 0.38*** & 0.37***  & $0.65^{.}$  \\
    \end{tabular}
    \label{category_color}
\end{table}

% Ranking related:  Order of Sentence Conclusions}
As shown in Table \ref{barRankCategoryORTable} and Figure \ref{fig:bar_all} annotation 4a+b, multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion rankings with conclusion categories suggests that people were most likely to make a main effect comparison first. Those who did not make a main effect comparison were more likely to have made a pair-wise comparison than anything else ($p_{interaction} = 0.002$, $p_{superlative} = 0.001$, $p_{other} < 0.001$). By the second conclusion, people were more likely to make a main effect comparison or a pair-wise comparison than other conclusions, but the likelihood of them making main effect comparison and pair-wise comparison were not significantly different ($p = 0.74$). By the third conclusion, people became more likely to make main effect comparisons again, and similar to what they did for the first conclusion, those who did not make a main effect comparison more likely made pair-wise comparisons ($p_{interaction} = 0.02$, $p_{superlative} = 0.004$, $p_{other} < 0.001$). Participants were not likely to make interaction comparisons, and when they did, it was mostly as their third conclusion, see Figure \ref{fig:bar_all} annotation 4c. More statistical details can be found in the supplementary materials.

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
\renewcommand{\arraystretch}{0.9}
  \caption{Bar Odds Ratio of Comparison Category by Order Compared}
  \begin{tabular}{llll}
  \newline \\ {\bf Category} & {\bf First Rank} & {\bf Second Rank} & {\bf Third Rank} \\ \hline 
 main effect & \textbf{1.00} &  \textbf{1.00} & \textbf{1.00} \\ 
 pair-wise & 0.38*** & \textbf{1.00} & 0.93 \\ 
 interaction & 0.12*** & 0.28*** & 0.48***\\
 superlative & 0.14*** & 0.17*** & 0.19*** \\ 
 others & 0.04*** & 0.10*** & 0.15*** \\
    \end{tabular}
    \label{barRankCategoryORTable}
\end{table}
















% Data Relation %
\subsection{Effect of Underlying Data Relation}
\label{dataRelationSection}
A $\chi^2$ test of independence with Bonferroni adjustment suggests that people more likely made main effect comparisons when they viewed data depicting one main effect and no interactions, or two main effects and no interactions, compared to data depicting an interaction but no main effects ($\chi^2 = 101.3$, $p < 0.001$), as shown in Figure \ref{fig:bar_relation} annotation 1. Post-hoc comparisons with Bonferroni corrections revealed that they were more likely to make pair-wise comparisons when viewing data depicting an interaction but no main effects ($z = 8.73$, $p < 0.001$), see Figure \ref{fig:bar_relation} annotation 2. Multinomial logistic regression analysis \cite{ripley2016package} predicting conclusion type with data relations further shows that people take into consideration the underlying data relation as they make comparisons of data. Table \ref{relation_color} shows the odds ratio of participants making a specific comparison for each of the three data relations, all using distal-group main effect comparisons as reference. We bolded the conclusion with the highest odds ratio for each color mapping per data relation.  % Overall, viewers were more likely to make main effect comparisons for data depicting one main effect and no interaction as well as for data depicting two main effects and no interaction. When they viewed data depicting no main effect but an interaction, they were equally likely to make main effect comparisons and pair-wise comparison at first, but shifting to make pair-wise comparisons more by their second and third conclusions.

\begin{table}[h]
\renewcommand{\arraystretch}{0.9} \small \centering
  \caption{Bar Odds Ratio of Data Relations by Color Mapping}
  \begin{tabular}{lllll}
  \newline \\ {\bf Data Relation} & {\bf Category} & {\bf No Mapping} & {\bf Incongruent} & {\bf Congruent} \\ \hline 
\multirow{6}{3.6em}{No Main Effect, Yes Interaction} & \rowcolor{gray!25} main distal & 1.00  & 1.00  & 1.00  \\
 & main proximal & 1.20  &  1.88  &  4.00**  \\
 & \rowcolor{gray!25} pair distal & $2.00^{\bullet}$ & 1.66 &  \textbf{5.40***}  \\
 & pair proximal & \textbf{2.60*}  &  \textbf{3.11**}  &  3.60* \\
 & \rowcolor{gray!25} int. distal & 0.00 & 0.44  & 0.00 \\
 & int. proximal & 1.10  & 1.11  &   2.20 \\ \hline 
 
 \multirow{6}{3.6em}{One Main Effect, No Interaction} & \rowcolor{blue!15} main distal &  1.00 & 1.00  & 1.00  \\
 & main proximal & \textbf{2.16**}  &  \textbf{2.58**}  & \textbf{4.00**}  \\
 & \rowcolor{blue!15} pair distal & 0.83  & \textbf{1.83}$^{\bullet}$  & 1.80  \\
 & pair proximal & 0.22**  &  1.08  &  0.50 \\
 & \rowcolor{blue!15} int. distal & 0.22** &  0.83 & 0.19* \\
 & int. proximal & $0.44^{\bullet}$ & 0.74  &  1.30 \\ \hline 
 
 \multirow{6}{3.6em}{Two Main Effects, No Interaction} & \rowcolor{gray!25} main distal & 1.00  & \textbf{1.00}  & 1.00 \\
 & main proximal & \textbf{1.10}  & 0.85  &  \textbf{1.23}  \\
 & \rowcolor{gray!25} pair distal & 0.37**  & 0.20***  &  0.23** \\
 & pair proximal & 0.24***  & 0.20***   &  0.42* \\
 & \rowcolor{gray!25} int. distal & 0.06*** & 0.28***  & 0.12*** \\
 & int. proximal &  0.10*** &  0.05*** & 0.12***  \\
    \end{tabular}
    \label{relation_color}
\end{table}

Specifically, viewers were more likely to make pair-wise comparisons when they see charts depicting no main effect but an interaction. Referencing Table \ref{relation_color} top section row 3 and 4, when the chart has no color-spatial mapping or incongruent color-spatial mapping, participants more readily made proximal-group pair-wise comparisons. When the chart had congruent color-spatial mapping, participants more readily made distal-group pair-wise comparisons. When the data depicted one main effect, but no interaction, viewers were more likely to make proximal-group main effect comparisons, see Table \ref{relation_color} middle section row 2. When the data depicted two main effects and no interaction, although not significantly, viewers more readily made proximal-group main effect comparisons for charts with no color mapping and congruent color-spatial mapping, and more distal-group main effect comparisons for charts with incongruent color-spatial mapping, see Table \ref{relation_color} bottom section row 1 and 2.

When we additionally consider the order in which the sentence conclusions were produced, for bar charts depicting \textit{an interaction but no main effect}, viewers seemed to start making comparisons by looking at the main effect or the pair-wise comparisons, as shown in Figure \ref{fig:bar_relation} top left grid. By the second conclusion, most viewers shifted to make pair-wise comparisons. %Amongst the pair-wise comparisons, people were the most likely to first make a proximal-group pair-wise comparison (and specifically, of the left group). Those who didn't make a proximal-group pair-wise comparison would likely make a proximal-group main effect comparison or a distal-group pair-wise comparison. For their second conclusion, they switch to make either a distal-group or a proximal-group pair-wise comparison of the right group. 
Very few participants made pair-wise proximity and edge comparisons (about 6\%), so we lumped them together as `others' in our figures. For those who did, these comparisons were often the second or third conclusion people drew, never the first. Notice there were few grey color patches in the top rows of Figure \ref{fig:bar_relation} (first conclusions), and more grey patches towards the bottom (third conclusions).

For bar charts depicting \textit{one main effect and no interaction}, the majority of conclusions were main-effect comparisons. People were the most likely to make proximal-group main effect comparisons as their first conclusion, as shown in figure \ref{fig:bar_relation} annotation 3a (note that size grouping is collapsed here). In fact, participants mostly made proximal-group main effect comparisons for their second and third comparisons as well. Those who didn't make main-effect comparisons mostly made pair-wise distal-group comparisons, although not as many people made pair-wise comparisons when viewing this data compared to data depicting no main effect but an interaction.

For bar charts depicting \textit{two main effects and no interaction}, people likely first made a proximal or distal main effect comparison. For their second conclusion, they either switched to make the other main effect comparison, or made a pair-wise comparison. Different from those who viewed bar charts depicting one main effect, participants who viewed bar charts depicting two main effects were equally likely to make distal-group and proximal-group pair-wise comparisons. 

\begin{figure}[h]
 \includegraphics[width=3.4in]{Figure/bar_relation.pdf}
 \caption{Conclusions by underlying data relations, aggregated across color mappings. The bar length presents the percentage of conclusions out of the total amount of conclusion per grid box (each grid box adds up to 100\%).}
 \label{fig:bar_relation}
\end{figure}

















% Size Grouping
%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[h]
 \includegraphics[width=17.8cm]{Figure/bar_size.pdf}
 \caption{Size grouping and proximal-group and distal-group conclusions made by viewers, with aggregated color mapping. The values in each cell indicate the percentage of conclusions in that category out of the total amount of conclusions for the column.}
 \label{fig:SizeGrouping}
\end{figure*}

\subsection{Effect of Size-Spatial Grouping}
\label{1asize}
Because underlying data relations (whether there exists main effect/interaction in the data or not) impacted the conclusions people drew, we also investigate the influence of size-spatial grouping of the marks, which is typically determined by the similarity of the underlying data values. We suspect that size-spatial grouping would serve as a better predictor to conclusions viewers make because it captures visual differences that collapsing over data relation does not. For example, the size-spatial congruent (tall tall short short) and incongruent (tall short tall short) versions of the one main effect no interaction chart are visually different. This difference is only captured when we look at size-spatial grouping, as they have the same underlying data relation.

We sorted the bar charts into four size-spatial grouping categories. As shown in Figure \ref{fig:SizeGrouping}, size grouping could be congruent with spatial grouping such that the two similarly large bars are spatially proximate, and the two similarly small bars are spatially proximate. An example of this category is the "one main effect, no interaction" chart that is grouped by company, see Figure \ref{fig:eightRelationships}(b). The second category is a variation that arranges the bars in decreasing size. An example of this category is the "two main effects, no interaction" chart that is grouped by region, see Figure \ref{fig:eightRelationships}(d). This decreasing grouping still maintains spatial-size congruency, such that the two larger bars are spatially proximate, and the two smaller bars are spatially proximate, but the bar sizes are not as similar as those in the first category. The third category is when size and spatial grouping are incongruent, such that the spatially proximate two bars significantly differ in size (tall short tall short). An example of this is the "one main effect, no interaction" chart grouped by region, see Figure \ref{fig:eightRelationships}(c). The fourth category is a variation that is also size-spatial incongruent where the tallest two bars are the furthest away from each other. Examples include the "no main effect, yes interaction" charts, see Figure \ref{fig:eightRelationships}(e)

People drew more proximal-group comparisons when size-spatial grouping is congruent, and more distal-group comparisons when size-spatial grouping is incongruent. As the size grouping become more incongruent with spatial grouping, people became more likely to draw a balanced amount of both proximal-group and distal-group conclusions. You can see that there were more orange (distal comparisons) moving from left (congruent size-spatial-grouping) to right (incongruent size-spatial grouping) in Figure \ref{fig:SizeGrouping} annotation 1. This shows a competition between spatial and size grouping, suggesting both drive what a viewer would conclude. If spatial grouping was always the stronger driver, you would expect participants to have always made proximal-group main comparisons. If size-grouping was the stronger driver, you would expect participants to have always made distal-group main comparisons when size-spatial grouping is incongruent. But this was not the case.

We observed similar dominance of main effect conclusions, with an increased number of pair-wise comparisons in incongruent polarizing charts, as shown in Figure \ref{fig:SizeGrouping} annotation 2+3. This makes sense as size-spatial grouping often depends on the underlying data relation, and incongruent polarizing charts are often depicting no main effects but an interaction, which suggests that size-spatial grouping is a better predictor than data relations as it captures the impact of data relations in a more nuanced way. Table \ref{size_color} shows the results of a  multinomial logistic regression analysis predicting conclusion type with size-spatial grouping. The likelihoods of participants drawing a particular conclusion under each size-spatial grouping were compared, using the likelihood of distal-group main comparison as reference (except for the incongruent color-spatial condition's congruent size-spatial column. No participant made distal-group main effect comparison when viewing the incongruent color-spatial chart, thus using distal-group main effect as a reference would result in exaggerated odds ratio). More details can be found in the supplementary materials. 

\begin{table}[h]
\renewcommand{\arraystretch}{0.9} \small \centering
  \caption{Bar Odds Ratio of Color Mapping by Size-Spatial Grouping}
  \begin{tabular}{llllll}
  \newline \\ {\bf Color} & {\bf Category} & {\bf Congru.} & {\bf Decreas.} & {\bf Incongru.} & {\bf Polariz.} \\ \hline
\multirow{6}{3em}{No Mapping} & \rowcolor{gray!25} main distal & 1.00 & 1.00 & \textbf{1.00} & 1.00 \\ 
 & main proximal  & \textbf{2.44*} & 1.46 & \textbf{1.20} & 1.20 \\
 & \rowcolor{gray!25} pair distal & $0.33^{\bullet}$ & 0.23* & 0.80 & $2.00^{\bullet}$ \\
 & pair proximal & 0.11* & \textbf{3.08*} & 0.24** & \textbf{2.60*} \\
 & \rowcolor{gray!25} int. distal & 5.00e-09 & 1.21e-08 & 0.24** & 2e-07 \\
 & int. proximal & $0.33^{\bullet}$ & 0.08* &  0.28** & 1.10 \\ \hline
 
  \multirow{6}{3em}{Incongr. Color Spatial} & \rowcolor{blue!15} main distal & 2.29e-07*** & 1.00 & \textbf{1.00} & 1.00 \\ 
 & main proximal & \textbf{1.00} & \textbf{$1.83^{\bullet}$} & 0.74 & 1.89 \\
 & \rowcolor{blue!15} pair distal & 0.62 &  $0.33^{\bullet}$ & 0.49* & 1.67 \\
 & pair proximal & 0.77 &  0.17* & 0.23*** & \textbf{3.11**}\\
 & \rowcolor{blue!15} int. distal & 0.31* & 0.25* & 0.37** & 0.44\\
 & int. proximal & 0.54 & 0.08* & 0.09*** & 1.11 \\ \hline
 
 \multirow{6}{3em}{Congr. Color Spatial} & \rowcolor{gray!25} main distal & 1.00 & 1.00 & \textbf{1.00} & 1.00 \\ 
 & main proximal & \textbf{26.0**} & \textbf{3.29**} & 0.82 & 4.00** \\
 & \rowcolor{gray!25} pair distal & 2.00 &  0.29 & 0.71 & \textbf{5.40***}\\
 & pair proximal & 4.00 & 0.57 & 0.29** & 3.60*\\
 & \rowcolor{gray!25} int. distal & 4.44 & $0.14^{\bullet}$ & 0.14*** & 5e-07*** \\
 & int. proximal & 1.10* & $0.14^{\bullet}$ & 0.14*** & 2.20\\
    \end{tabular}
    \label{size_color}
\end{table}

As shown in Table \ref{size_color} top section, for charts with \textit{no color mapping}, viewers were most likely to make proximal-group main comparisons when they saw congruent size-spatial grouping charts, 2.44 times that of making a distal-group main comparison, and significantly more than other comparison types. Viewers were the most likely to make proximal-group pair-wise comparisons when they saw congruent decreasing charts, equally highly likely to make proximal- and distal-group main effect comparisons when they saw incongruent size-spatial grouping charts, and most likely too make proximal-group pair-wise comparisons when viewing incongruent polarizing charts. For charts with \textit{incongruent color-spatial mapping}, viewers were most likely to make proximal-group main effect comparisons when viewing congruent size-spatial charts, slightly more likely to make proximal-group main effect comparisons when they saw decreasing charts, equally likely to make proximal- and distal-group main effect comparisons when they saw incongruent size-spatial grouping charts, and most likely to make proximal-group pair-wise comparisons when they saw incongruent polarizing charts. For charts with \textit{congruent color-spatial mapping}, viewers were most likely to make proximal-group main effect comparisons when viewing congruent size-spatial charts and congruent decreasing charts, equally highly likely to make proximal- and distal-group main effect comparisons when they saw incongruent size-spatial grouping charts, and more likely to make distal-group pair-wise comparisons when viewing incongruent polarizing charts. 

% We see that the patterns of how sentence conclusions and distal/proximal comparisons made in the congruent decreasing column and the incongruent size-spatial grouping column are very similar. This makes sense because although they depict different underlying data relations, the similar size grouping makes the two size-grouping look visually similar. This likely  guided the viewers to form similar visual groups and thus generated similar sentences. Further, in the left chart in Figure \ref{fig:SizeGrouping}, comparing across the three horizontal sections with different color mapping, we see that the distribution of sentence conclusions in each category across the four size groupings, as well as the distal-proximal ratio (purple-orange ratio), does not look significantly different. This further supports the previous analysis showing that color grouping does not seem to play a major role in driving viewer conclusions overall. 
Although color grouping has a weak effect on comparisons, we did see an effect of of color on comparisons made when the size-grouping is \textit{incongruent polarizing} (see right-most column, the middle and bottom sections in Table \ref{size_color}). When the chart had incongruent color-spatial grouping, participants more readily made \textit{proximal-group} pair-wise comparisons, 3.11 times that of main distal comparisons, but when the chart had congruent color-spatial grouping, participants more readily made \textit{distal-group} pair-wise comparisons, 5.40 times that of main distal comparisons. 

Overall, the effects of size-spatial grouping seemed to be more granular and able to account for the effect of data relation, suggesting that size grouping is a more effective predictor guiding viewer conclusions. Next, we examine potential interactions between color- and size-spatial grouping on comparisons made.












% Interaction distal Size, Data Relation, and Color
%%%%%%%%%%%%%%%%%%%%%
\subsection{Interaction between Color, Size, and Spatial Grouping}
We compared the odds ratio of participants comparing the \textit{two spatially proximate groups} for each color mapping, across the four possible size-spatial groupings, as shown in the top section of Table \ref{color_size_spatial}, using no color mapping as reference. Overall, besides that viewers were more 1.57 times more likely to make proximal comparisons when viewing congruent size-spatial charts with congruent color-spatial mapping, everything else was approximately equal. The middle section documents the odds ratio of participants comparing the \textit{two distal groups}. Again, besides that viewers were only a quarter as likely to make distal comparisons when viewing congruent size-spatial charts with congruent color-spatial mapping, everything was approximately equal. This again suggests that color had negligible effects on guiding comparisons. 

The bottom section directly compares the odds ratio of participants making a proximal- versus a distal-comparison across size-spatial groupings, collapsing over color-spatial grouping. This serves as a proxy to estimate and compare the effect of spatial and size grouping on sentence conclusion generations. For instance, larger likelihoods of making proximal comparisons suggests a stronger effect of spatial grouping on eliciting comparisons. Participants were more likely to make proximal comparisons overall. They were approximately twice as likely to make proximal comparisons, and half as likely to make distal when they viewed congruent size-spatial charts and incongruent polarizing charts. This pattern flipped for when participants viewed incongruent size-grouping charts. When they viewed congruent decreasing chart, they were equally likely to make proximal- and distal-comparisons.

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{Bar Odds Ratio Aggregated Color, Size, and Spatial Grouping}
  \begin{tabular}{lllll}
  \newline \\ {\bf Proximal Comparisons} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\ 
  \hline 
 No Color Mapping & 1.00 & 1.00 & 1.00  & 1.00  \\
 Color-Spatial Incongru. & 1.15 & 1.04 & 0.86  &  1.12 \\
 Color-Spatial Congru. & 1.57* & 1.16  & 0.81 &  1.00 \\
 
 \newline 
 \newline \\ {\bf Distal Comparisons} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\ 
  \hline 
 No Color Mapping & 1.00 & 1.00 & 1.00  & 1.00  \\
 Color-Spatial Incongru. & 0.99  & 1.18 & 1.27  &  0.93  \\
 Color-Spatial Congru. &  0.24* &  0.63  & 1.01  & 1.07   \\
 
 \newline \rowcolor{white}
  \newline  \\ {\bf Total} & {\bf Congru.} & {\bf Decreasing} & {\bf Incongru.} & {\bf Polarizing} \\
 \hline 
 \rowcolor{gray!25} proximal & 2.11** & 1.00 & 0.40*** & 1.70***  \\
 \rowcolor{white} distal & 0.47**  & 0.99 & 2.48***  & 0.59***   \\
 
    \end{tabular}
    \label{color_size_spatial}
\end{table}

















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Bar Visualization Conclusion}
In general, viewers are the most likely to make main effect comparisons. They made pair-wise comparisons more readily when the underlying data is depicting an interaction but no main effect, or when the size-spatial grouping is incongruent and polarizing (these patterns tend to co-occur, see Figure \ref{fig:eightRelationships}(e). Viewers rarely generated interaction comparisons, even when the underlying data was showing only an interaction with no main effects. When viewers saw this type of charts, they made pair-wise comparisons between spatially adjacent data values.
Surprisingly, varying color mapping in bar visualizations had only a small impact on what comparisons a viewer would make. There was one exception, where color influenced which pair-wise comparison a viewer would make when the data depicted an interaction but no main effect, such that incongruent color-spatial arrangements increased the likelihood of viewers making proximal pair-wise comparisons. On the other hand, size-spatial grouping have a much bigger impact on guiding viewer conclusions. Overall, viewers are approximately 31\% more likely to generate sentence conclusions comparing spatially proximate data values than spatially separated ones, and this tendency can be doubled or halved depending on the size-spatial grouping. 



==> Old_Text/future.tex <==
%% LIMITATIONS AND FUTURE DIRECTIONS %%
\section{Summary}
Overall, viewers were the most likely to make main effect comparisons. When viewing bar charts, they made pair-wise comparisons more readily when the underlying data depicted no main effect but an interaction, or when the data was organized with polarizing incongruent size-spatial grouping (they tend to co-occur, as shown in Figure \ref{fig:eightRelationships}(e)). They rarely generated interaction comparisons, even when the underlying data showed only an interaction with no main effects, corroborating findings in psychology suggesting that interaction is cognitively difficult to discern and express \cite{halford2005many, shah2011bar}. Varying color mapping in bar visualizations had a negligible impact on what comparisons a viewer would make. There was a competition between size- and spatial-grouping, such that viewers were approximately 31\% more likely to generate sentence conclusions comparing spatially proximate data values than spatially separated ones, and this tendency could be doubled or halved depending on the size-spatial grouping. In multi-class scatterplots, color was more likely to be compared first than shape, but by the third conclusion, shape became more likely to be compared. 

\section{Limitations and Future Directions}
\label{limitation}
We relied on a particular set of underlying data values to serve as a case study for the entire space of 2x2 bar charts, which subsequently serves as a case study of the entire space of bar charts, across number of points, the shape of the data table, and more global aspects of data arrangement (e.g. interleaved vs. small multiple designs \cite{jardine2019perceptual}). We tested an equivalently small space for scatterplots in Experiment 2. Clearly, more work will be needed to confirm how far the results found in these smaller worlds will extrapolate to bigger ones. 

There are other grouping features to test, as well. Using more powerful divisions among shape marks, such as open vs. closed shapes \cite{burlinson2017open}, or weaker color cues \cite{szafir2017modeling} might lead shape to rival or beat color categories in a new version of our scatterplot experiment. Just as size-spatial grouping proved to be an important factor for the bar chart experiment, despite being driven by the data alone, we might expect other similarities in data marks -- perhaps lines of the same orientation, or heatmap values with a similar color -- to be similarly more heavily weighted as groups. 

The present work attempted to ignore the viewer's goals and omitted titles, annotation, and any other context that might guide comparison, in order to maximally isolate the impact of the graph design. These factors are important, and future work could assess their influence against that of the chart's design. It would be especially important to measure graphical literacy as a potential mediator of that relationship. Similarly, we found a trend for comparisons to proceed in a `left-to-right' order, such that pairwise comparisons of the two left bars were prioritized over the same comparison of the two right bars. While this trend matches with a general left-to-right bias for human attention \cite{michal2017visual, holmqvist2005role, zacks2001event}, our leftmost bars were also more likely to be taller, so the present design does not allow examination of that trend deconfounded from other salient cues. 

The verbal description method is inspired by a literature on `sentence-picture congruity' from psychology \cite{clark1972process}, and we use it as a proxy for the visual comparison that was most salient to a viewer. However, future work might seek converging evidence from other measures, such as what comparisons people remember after a brief viewing, what changes to data values they notice, or what decisions they make based on the data. 

Our dataset comprises hundreds of verbal descriptions of visualizations. This dataset could be expanded in both volume and scope of visualization types, and text descriptions could be augmented with automated mining of existing descriptions. If a natural-language processing algorithm (or crowdworkers) could be leveraged to turn these descriptions into the type of expressions shown in Table \ref{pilot_equation}, and the visualizations could be discretized into qualitative descriptions, (e.g. Vega \cite{satyanarayan2016vega}), the combined dataset could become the input that trains a more comprehensive prediction engine for what comparisons are made by a typical visualization viewer.

\section{Guidelines and Conclusions}
For a bar chart, place the values that your audience should compare (or treat as a group) next to each other. Making them different colors may not hurt, but the added benefit is likely minimal. Beware that viewers are likely to group values of similar sizes, whether or not they should do so. For a scatterplot, your viewers will prioritize comparing different colors over shapes.  

Most current work on visual comparison focuses on the efficiency or precision of a given comparison. We argue that these factors are important, but irrelevant if a visualization viewer never makes that comparison in the first place. In our real-world experience, the biggest delays in understanding a new visualization are knowing how to read a visualization and knowing which patterns one should pay attention to. When communicating data, analysts tend to assume that the viewer sees what they see \cite{xiong2019curse}, instead of designing the visualization to push the viewer toward seeing the `right' pattern. We hope that refinement of the type of model developed here can lead to a set of guidelines or concrete tools to help them achieve that goal. 




==> Old_Text/pilotOLD.tex <==

We first tested whether crowdworkers on Amazon's Mechanical Turk (MTurk) could produce typed responses that we could interpret to confidently assess the comparison that they found most salient. We showed 58 participants bar charts through Qualtrics on MTurk \cite{snow2013qualtrics}. Participants viewed a bar chart depicting the revenues of two companies in two regions, as shown in the left-most chart in Figure \ref{fig:teaser}. The underlying data comprises a 2x2 factorial design - two levels of company (A and B) and two levels of region (East and West). It illustrated a main effect of company (revenue of A is greater than that of B), a main effect of region (revenue in the West is greater than that in the East), and an interaction between company and region. In the experiment, the bars could either be spatially grouped by company (see first chart in Figure \ref{fig:teaser}) or by region (see second chart in Figure \ref{fig:teaser}).

Participants were prompted to type the first conclusion they would draw from the chart. After typing the first conclusion, a new prompt would appear on the same page and ask them to enter the second conclusion. This continued until the participant entered five conclusions. Then, on a separate page, they entered demographic information such as their age and gender. The order in which they wrote the sentence conclusions were recorded as the sentence rankings. The effect sizes obtained from these results were also used to determine the sample size needed for Experiment 1. 

All responses were transformed into expressions by two human coders and categorized following the taxonomy above. These expressions categorize the human sentences into common comparisons in data. We discuss the potential of using this coding system for creating recommendation systems in Section \ref{limitation}. Table \ref{pilot_equation} summaries the taxonomy, giving examples of responses, expressions and comparison categories.

\subsection{Insights from Pilot}
\label{insightFromPilot}
We noticed that several participants mentioned multiple comparisons in the same conclusion. For example, when prompted to report the first conclusion, the participant identified both a distal-group pair-wise comparison and a proximal-group pair-wise comparison. In these cases, we broke up the response in two parts and included each in its corresponding categories, preserving the rank order for both. We also noticed that many participants stopped giving interpretable answers after the third conclusion, typing answers such as "I can't draw any additional conclusions." We therefore limited the total number of comparison prompts to three.  

The underlying data chosen for the pilot includes both main effects and an interaction, but we observed very few conclusions mentioning interactions. This may reflect interactions being cognitively more difficult to extract, but it also could be due to the particular data values used in the pilot. For the main experiment we therefore decided to sample other possible datasets for the 2x2 factorial visualizations. We also noticed that people tended to be guided by size-spatial grouping, such as whether a tall bar is spatially grouped with another tall bar, versus a short bar. Because size-spatial grouping depends on the values in the dataset, this factor is intertwined with the previous challenge of choosing new sets of data values. 

Figure \ref{fig:eightRelationships} depicts eight possible categories of datasets, depending on whether there exist main effects and/or interactions. Note that size grouping can be congruent or incongruent with spatial grouping, as shown in (b) and (c), respectively.

%% Eight Relationships of Main Effects and Interactions %%
\begin{figure}[th]
 \includegraphics[width=3.4in]{Figure/AllEightRelationships.jpg}
 \caption{Eight possible relations of two two-level factors. Note that the outcomes are idealized examples; perfect outcomes rarely occur in actual data. % The top four visualizations depict outcomes in which there is no company x region interaction, and the bottom four visualizations illustrate outcomes in which there is. The columns vary in presence and location of main effects in the data. 
 Blue colored ones are examined in depth in this paper.}
 \label{fig:eightRelationships}
\end{figure}



%% Bar Visualization Design Space%%
\begin{figure}[bh]
 \includegraphics[width=3.4in]{Figure/BarDesignSpace.pdf}
 \caption{Design space for bar visualization experiment. These are the three data relations used for this experiment, chosen from the set of relations depicted in Figure \ref{fig:eightRelationships}. The first row shows no color mapping, the second row shows incongruent color-spatial mapping, and the third row shows congruent color-spatial mapping.}
 \label{fig:exp1design}
\end{figure}

==> Old_Text/scatterplot_exclude_.tex <==
%% EXPERIMENT 2 %%
\section{Experiment 2: Scatterplot Visualizations}
The previous investigation of bar charts revealed a grouping strength ranking of spatial first, size second, and color third. 
%Another popular encoding channel in visualization, shape, has not yet been considered. While it's difficult to manipulate shape in bar visualizations beyond changing aspect-ratio of bars, 
Experiment 2 compared two other grouping cues -- color versus shape -- in scatterplots.
%provide an suitable testing ground to further investigate the effect of shape as a grouping cue to elicit conclusions. 
We followed the two binary factor setup in the bar visualization experiment and created scatterplots visualizing the performance of two types of car engine (straight and v-shaped) on quarter mile time and fuel economy for two transmission types (automatic and manual). 

Similar to the bar experiment, participants viewed scatterplots and typed the top three conclusions they would draw. We tested four configurations of the scatter plots, as shown in Figure \ref{fig:scatterDesignSpace}. We used the mtcars dataset, identified two factors - engine and transmission, which are encoded either with color (default ggplot teal #00BFC4 and red #F8766D) or shape (default circle or triangles) - and plotted their corresponding fuel economy and quarter mile time. We crossed the color and shape encodings, and counterbalanced the x- and y-axes to produce the four configurations: two have engine encoded using color, and two have transmission encoded using color; two have quarter mile time plotted on the x-axis, and two have fuel economy plotted on the x-axis. Participants were excluded following the same exclusion criteria as Experiment 1. We excluded 2 participants and 11 nonsensical or empty responses, and are left with 69 participants ($MeanAge = 39.2$, $SD = 11.31$, $23$ females) and 202 conclusions.

\begin{figure}[ht]
 \includegraphics[width=3.4in]{Figure/ScatterPlotStimulus.jpg}
 \caption{Above are the scatterplot stimuli used in Experiment 2, depicting two factors encoded with color or shape. The same data was presented and counterbalanced with which factor was encoded to which channel (color or shape) as well as switching of the x and y variables.}
 \label{fig:scatterDesignSpace}
\end{figure}









%% Comparison Categorization %%
\subsection{Response Categorization} 
We categorized the conclusions participants made from the scatterplots following a similar taxonomy as the bar chart experiment. Participants drew main effects and pair-wise comparisons, and identified superlatives. The scatterplot format also enabled participants to draw additional categories of conclusions, including correlations and distributions. No one compared interactions between any of the factors.

\textbf{Main Effects:}
We categorized conclusions comparing how each factor performed on either the x- or y-axis as a main effect comparison. Comparing manual to automatic transmission or straight to v-shaped engine performance on either axis (quarter mile time or fuel economy) are main effect comparisons. These comparisons could happen either using color or shape grouping. For instance, if manual transmissions were colored red and automatic transitions were colored blue, concluding "manual transmissions have a faster quarter mile time than automatics" would be a color comparison. If transmission were encoded by shape instead, the previous example would be a shape main effect comparison.

\textbf{Pair-Wise Comparisons:}
Conclusions comparing one level of a factor while keeping the levels of the other factor constant is categorized as pair-wise conclusions. These comparisons can be across color or across shape. For instance, "V-shaped engines with manual transmissions are slower than straight engines with manual transmissions." For the condition in which engines were assigned shape, this would be an across-shape comparison, comparing two shapes across the same color. For the condition in which engines were assigned color, this would be an across-color comparison, comparing different colors across the same shape. Therefore, a pair-wise comparison counts towards both color and shape. % When making this type of comparison, the viewer takes into account one dimension of the dataset (shape or color). They also then take into account the other dimension in the comparison itself. So, in the previous example, both engine type and transmission type are mentioned, indicating that both color and shape are considered. 

\textbf{Superlatives:}
Some participant conclusions were about the single best performing combination of engine and transmission. For example, a participant concluded, "A straight manual transmission will give you the highest fuel economy." Unique to the scatterplot condition, some superlative codes were about performance in the x-axis, while some were about performance in the y-axis, and some were about overall performance across both axes. In this example, because the participant mentioned both engine (straight) and transmission (manual), we consider it as having mentioned both color and shape. 

\textbf{Correlations:}
Participants also commented on the relation between the x- and y-axes. Conclusions in this category often included descriptions of a correlation between fuel economy and quarter mile time. "The faster the car, the more fuel economy it gets" is an example that indicated the viewer's understanding of the general positive trend in the data. 
% \textbf{MEOW: I don't get the rest of this para: This is still a comparison, just diff from what you are studying. Just say it's diff and you'll note it but not discuss in detail?} However, this type of conclusion does not indicate any comparisons being made, as neither transmission type nor engine type matter when determining the overall trend of the data. So, the viewer here doesn't consider either dimension. \textbf{MEOW:??}

\textbf{Distributions:}
This category included any conclusion that centered around the spread of the data rather than the performance differences between factors. It contains three sub-categories: count, range, and variation. Count pertains to the number of each factor. For instance, "there are more V-shaped than straight engines." %which would have been a main effect comparison if it had centered around performance rather than number of data points. 
Range mentions the performance of the data points but makes a value statement, rather than a comparison, such as "there are no engines that are over 35 [miles per gallon] for fuel economy." While this mentions the performance of engines, there are no comparisons being made. Instead, the conclusion refers again to the spread of the data. Variation is about data variability, such as "V-Shaped manuals seem to perform consistently." % This conclusion is not making a comparison, similar to the previous subcategories, but rather an observation about the spread of the data. However, it does not fall into the subcategory of "range," since there are no value-based observations. Unlike the correlation category, conclusions in this category do consider the dimensions of data. In the count example, the viewer considers engine type but not transmission type, so they examine either one color or one shape. In both the range and variation examples, the viewers mention performance of a specific dimension of data. So, despite not making direct comparisons of the data groups, the responses here still indicate considerations and some understanding of the different dimensions. 

















\begin{figure}[th]
 \includegraphics[width=3.4in]{Figure/scatter.pdf}
 \caption{Comparison category by features compared in scatterplots. Top row shows the distribution of people comparing color versus shape for main effects. Bottom two rows show stacked distribution of features compared (color, shape, both, neither) for other categories. Bar length shows the number of comparisons made in a specific category out of all comparisons made for that rank. Error bars show standard error. }
 \label{fig:scatter}
\end{figure}

%% Results %%
\subsection{Sentence Conclusions for Scatterplots}
Overall, viewers most likely drew main effect conclusions (68.3\%), followed by superlative conclusions (15.3\%), distribution conclusions (6.9\%), pair-wise conclusions (5.0\%), and least likely correlations (4.5\%). Table \ref{scatter_rank_category} shows the odds ratio of a particular category of conclusion being drawn for each rank order, using main effect conclusion as reference. Similar to that in bar charts, participants were significantly more likely to make main effect comparisons across all three conclusions they made. For example, looking at the top table column for the `First' rank, pair-wise comparisons were only 2\% as likely to be mentioned as the first conclusion compared to main effects. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{Scatterplot Odds Ratio of Comparison Category and Order Compared}
  \begin{tabular}{llll}
  \newline \\ {\bf Conclusion} & {\bf First} & {\bf Second} & {\bf Third} & \hline 
 main effect & 1.00 & 1.00 & 1.00 \\
 pair-wise & 0.02*** &  0.09*** & 0.12***\\
 superlative & 0.22*** & 0.25*** & 0.21***\\
 correlation & 0.08*** & 0.09*** & 0.02*** \\
 distribution & 0.04*** & 0.07*** & 0.37*** \\ 
  \newline
  \newline \\ {\bf Comparison} & {\bf First} & {\bf Second} & {\bf Third} & \hline 
 compare color & \textbf{1.00} & \textbf{1.00} & 1.00 \\
 compare shape & 0.26*** & 0.38** & \textbf{1.28}\\
 mention both & 0.28*** & 0.38** & 0.86 \\
 mention neither & 0.07*** & 0.03*** & 0.05**\\
    \end{tabular}
    \label{scatter_rank_category}
\end{table}

Participants were more likely to compare color as their first and second comparison, see Figure \ref{fig:scatter} annotation 1 and Table \ref{scatter_rank_category} bottom section. A majority of people shifted to compare shape or mentioned both color and shape by their third comparison, as shown in Table \ref{scatter_rank_category} and Figure \ref{fig:scatter} annotation 2. More specifically, as shown in the bottom of Table \ref{scatter_rank_category}, viewers compared shape only 0.26 times as likely as they compared color in the first sentence conclusion. But by the third sentence conclusion they generated, they became 1.28 times more likely to compare shape relative to comparing color. In multi-class scatterplots we tested, color and shape are salient features such that very few people generated sentences without mentioning either color or shape. 

\begin{table}[h]
\rowcolors{2}{gray!25}{white} \small \centering
  \caption{Scatterplot Odds Ratio of Category and Features Compared}
  \begin{tabular}{lllll}
  \newline \\ {\bf Conclusion} & {\bf Color} & {\bf Shape} & {\bf Both} & {\bf None} \\ \hline 
 main effect & 1.00 & 0.51***  & 0.00*** & 0.00  \\
 pair-wise$^1$ & 1.00 & 0.00  & 0.00 & 1.26e+41*** \\
 superlative & 1.00 & 0.00*** & 30.00*** & 0.00***  \\
 correlation & 1.00 & 1.00 & 0.00 & 2.50   \\
 distribution &  1.00 & 0.43 &  0.57 & 0.00  \\
    \end{tabular}
    \label{category_compared_scatter}
\end{table}

As shown in Table \ref{category_compared_scatter}, overall color was the most compared feature across all categories. Viewers were half as likely to compare shape when making main effect comparisons. When viewers made pair-wise comparisons\footnote{The low-N in the pair-wise comparison category created super large and super small odds ratios.}, because this relied on selecting one dimension (either color or shape) and comparing how the levels of the other dimension differed on the selected dimension, both color and shape must have been mentioned. This resulted in a skewed, large odds ratio in the `Both' column. While there were only 10 conclusions that were pair-wise comparisons in our data, eight of them compared the two groups with different shapes of the same color, while only two compared the two groups of the same shape with different colors. While there were not enough data points to make reliable statistical inferences, it seemed to support the previous analysis that color was a stronger grouping cue than shape. We expand on this observation in Section \ref{limitation} to further discuss potential implications. 

We also examined whether viewers more readily compared visual groups based on the x- or y-axis value. Chi-squared test for given probabilities comparing the number of times people made x- or y- axis based comparisons suggested that, with post-hoc bonferroni adjustmets \cite{herve2020package}, people were equally likely to compare values on the x- and y-axis ($\chi^2 = 63.72$, $p_{xy(posthoc)} = 1.00$).

% \begin{figure}[th]
%  \includegraphics[width=3.4in]{axis_scatter.jpg}
%  \caption{People more likely to compare things based on the y-axis value.}
% \label{fig:scatter_xy}
% \end{figure}

%% Quant %%
% \subsection{Scatterplot Conclusion}
% In bar visualizations, we found color to have relatively weak influence in guiding viewer conclusions from data. Further investigation of the effect of color suggests that color was more likely to be compared first than shape in multi-class scatterplots. Similar to bar visualizations, viewers were significantly more likely to extract main effect comparisons, and they were just as likely to compare visual groups based on the x- and the y-axis variable.




==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
last modified by Bernhard Finkbeiner, July 5, 2010

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored by
the IEEE Visualization & Graphics Technical Committee (VGTC).

The only conferences that use the 'journal' document option:
- IEEE Visualization Conference (Research and Application Papers Only)
- IEEE Information Visualization Conference (Research and Application
Papers Only)

It contains 13 files:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed,
                  somewhere in the TeX search path
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
sample.eps      - an image used by the example paper
sample.pdf      - its PDF version
template-journal*.pdf    - an example proper pdf output in default
                          conference mode, with and without teaser
CypressView.eps - teaser image
CypressView.pdf - its PDF version
makefile     - makefile including bibtex compilation and proper PDF
                generation

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We
suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create
a file called 'template.pdf'. Please make sure, that its layout is
identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process
manually.  Below are a list of available options that may be passed to
make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> pilot.tex <==
We conducted a pilot study using crowdsourcing with two goals in mind: first, we wanted to test whether crowdworkers on Amazon's Mechanical Turk (MTurk) could produce verbal sentence responses that we could interpret to confidently assess which comparison type they made. Second, we wanted to see if our taxonomy based in existing psychology and cognitive science literature covers the comparisons people make. To do this, we showed 58 participants bar charts through Qualtrics on MTurk \cite{snow2013qualtrics}. Participants viewed a bar chart depicting the revenues of two companies (A and B) in two regions (East and West), similar to the ones shown in Table \ref{comparisonTypes}. 

% as shown in the left-most chart in Figure \ref{fig:teaser}. The underlying data comprises a 2x2 factorial design - two levels of company (A and B) and two levels of region (East and West). It illustrated a main effect of company (revenue of A is greater than that of B), a main effect of region (revenue in the West is greater than that in the East), and an interaction between company and region. In the experiment, the bars could either be spatially grouped by company (see first chart in Figure \ref{fig:teaser}) or by region (see second chart in Figure \ref{fig:teaser}).

Participants were prompted to type the first conclusion they drew from the chart. After they typed their first conclusion, a new prompt appeared on the same page and asked them to enter a second conclusion. This continued until the participant entered five conclusions. Then, on a separate page, participants entered demographic information such as their age and level of education. The order in which they wrote the conclusions was recorded as the sentence \textit{ranking}. 

All responses were interpreted by two human coders and categorized following the taxonomy in Table \ref{comparisonTypes}. While detailed results from the pilot can be found in the supplementary materials, we discuss some insights we gained from the pilot that helped us finalize our experimental designs. We discuss the potential of using this coding system for creating recommendation systems in Section \ref{limitation}. 

\subsection{Insights from the Pilot}
\label{insightFromPilot}
We noticed that several participants mentioned multiple comparisons in the same conclusion. For example, when prompted to report the first conclusion, the participant identified both a group comparison and a pair comparison. In these cases, we broke up the response in two parts and included each in its corresponding category, preserving the rank order for both. We also noticed that many participants stopped giving interpretable answers after the third conclusion, typing answers such as "I can't draw any additional conclusions." We therefore limited the total number of comparison prompts to three for our experiments.

Additionally, we observed that very few conclusions were second order comparisons \andrew{Is this talking about second-order quantitative only?}. This may reflect second-order comparisons being cognitively more difficult to extract, but it also could be due to the particular data values used in the pilot. For the our main experiments, we therefore decided to create three different datasets. This will not only help us generalize our findings across different datasets, but also shed light on whether the underlying relationship between the data values shown in the bar chart would affect the types of comparisons viewers make. 

\andrew {This paragraph would be more informative if we said something about how the three datasets differ from each other, and from the pilot dataset.} 
\cx{fully describe the motivation for creating the three different datasets, and describe how they are different here!}

Some participants in the pilot also gave responses that didn't fall in the categories defined in Table \ref{comparisonTypes}. These typically included comments about the number of companies shown, the colors used in the visualization, or axis-labels. We decided to include an additional category of \textit{Other} to capture these conclusions. Furthermore, some participants commented on implications, novelty or "obviousness" of data, such as saying "I would invest in company A in the future." Following the approach taken in \cite{shah2011bar} for similar responses, we included conclusions like these in the \textit{Other} category as well.

